Influence Minimization via Blocking Strategies

We study the influence minimization problem: given a graph $G$ and a seed set $S$, blocking at most $b$ nodes or $b$ edges such that the influence spread of the seed set is minimized. This is a pivotal yet underexplored aspect of network analytics, which can limit the spread of undesirable phenomena in networks, such as misinformation and epidemics. Given the inherent NP-hardness of the problem under the IC and LT models, previous studies have employed greedy algorithms and Monte Carlo Simulations for its resolution. However, existing techniques become cost-prohibitive when applied to large networks due to the necessity of enumerating all the candidate blockers and computing the decrease in expected spread from blocking each of them. This significantly restricts the practicality and effectiveness of existing methods, especially when prompt decision-making is crucial. In this paper, we propose the AdvancedGreedy algorithm, which utilizes a novel graph sampling technique that incorporates the dominator tree structure. We find that AdvancedGreedy can achieve a $(1-1/e-\epsilon)$-approximation in the problem under the LT model. Experimental evaluations on real-life networks reveal that our proposed algorithms exhibit a significant enhancement in efficiency, surpassing the state-of-the-art algorithm by three orders of magnitude, while achieving high effectiveness.

==> IMIN-IC.tex <==
We also show that the function of expected spread under IC model is monotone and not supermodular. 

\begin{theorem}
Given a graph $G$ and a seed set $S$, the expected spread function $\mathbb{E}(S,G[V \setminus B])$ under IC model is monotone and not supermodular of $B$.
\label{theo::expectedspread}
\end{theorem}


\begin{proof}
%As the interpretation of expected spread with IC model presented in Lemma~\ref{lemma:sample}, vertex blocking will remove the blocker from the sample graphs, thus the number of vertices that seeds can reach will not increase in any sample graphs, which means 
As adding any blocker to any set $B$ cannot increase the expected influence spread, we have $\mathbb{E}(S,G[V \setminus B])$ is monotone of $B$.
% For every two set $X\subseteq Y\subseteq V$ and vertex $x\in V\setminus Y$, if function $f(\cdot)$ is submodular, it must hold that $f(X\cup \{x\})-f(X)\ge f(Y\cup \{x\})-f(Y)$. Let $f(B)=\mathbb{E}(S,G[V \setminus B])$, $X=\{v_4\},Y=\{v_4,v_5\}$ and $x=v_2$, In Figure~\ref{fig:sample}, we have $f(X)=6.66$, $f(Y)=2$, $f(X\cup \{x\})=1$, $f(Y\cup \{x\})=1$, therefore $f(X\cup \{x\})-f(X)=-5.66 < f(Y\cup \{x\})-f(Y)=-1$. $\mathbb{E}(S,G[V \setminus B])$ is not submodular of $B$.
For every two set $X\subseteq Y\subseteq V$ and vertex $x\in V\setminus Y$, if function $f(\cdot)$ is supermodular, it must hold that $f(X\cup \{x\})-f(X)\le f(Y\cup \{x\})-f(Y)$. 
Consider the graph in Figure~\ref{fig:sample}, let $f(B)=\mathbb{E}(S,G[V \setminus B])$, $X=\{v_3\},Y=\{v_2,v_3\}$ and $x=v_4$. As $f(X)=6.66$, $f(Y)=5.66$, $f(X\cup \{x\})=5.66$, and $f(Y\cup \{x\})=1$, we have $f(X\cup \{x\})-f(X)=-1 > f(Y\cup \{x\})-f(Y)=-4.66$.
\end{proof}

In addition, we prove that the IMIN problem is hard to approximate.

\begin{theorem}
The IMIN problem is APX-hard unless P=NP.
\label{theo::APX}
\end{theorem}

\begin{proof}
We use the same reduction from the densest k-subgraph (DKS) problem to the Influence Minimization problem, as in the proof of Theorem~6.
Densest k-subgraph (DKS) problem does not have any polynomial-time approximation scheme, unless P=NP~\cite{Khot06}.
According to the proof of Theorem~6, we have a blocker set $B$ for influence minimization problem on $G'$ corresponding to a vertex set $A$ for DKS problem, where each $c_i\in B$ corresponds to $v_i\in A$.
Let $x$ denote the number of edges in the optimal result of DKS, and $y$ denote the optimal spread in IMIN, we have $x+k=y$, where $k$ is the given positive number of DKS problem.
If there is a solution with $\gamma$-approximation on the influence minimization problem, there will be a $\lambda$-approximation on the DKS problem.
Thus, there is no PTAS for the influence minimization problem, and it is APX-hard unless P=NP.
\end{proof}

==> appro.tex <==
\section{Existing works and our approach for IMIN problem}
\label{sec:appro}

The hardness of the problem motivates us to develop an effective and efficient heuristic algorithm. 
In this section, we first introduce the state-of-the-art solution (i.e., the greedy algorithm with Monte-Carlo Simulations) as the baseline algorithm (Section~\ref{sec:baseline}). Then, we analyze existing solutions for expected spread computation, and propose a new estimation algorithm based on sampled graphs and dominator trees to compute the decrease of expected spread for all vertices at once (Section~\ref{sec:candidates}). Applying the new framework of expected spread estimation for selecting the candidates, we propose our AdvancedGreedy algorithm (Section~\ref{sec:advanced-greedy}) with higher efficiency and without sacrificing the effectiveness, compared with the baseline.
As the greedy approaches do not consider the cooperation of candidate blockers during the selection, some important vertices may be missed, e.g., some out-neighbors of the seed.
 %and we have to block all the out-neighbors of the seeds for influence minimization with a large budget.
Thus, we further propose a superior heuristic, the GreedyReplace algorithm, to achieve a better result quality (Section~\ref{sec:greedyreplace}).


% In this section, we firstly show the existing solutions for computing expected spread are infeasible for solving the influence minimization problem, and propose the Iterative Progress algorithm (Section~\ref{sec:expspcal}).
% For the computation of blocker set, existing studies focus on greedy approaches to select the resulting blockers while the cooperation of candidate blockers is not considered \cite{min-greedy1,min-greedy-tree,min-greedy2}.
% Thus, we first propose the Release algorithm to consider blocker cooperation by focusing on the out-neighborhood of the seeds (Section~\ref{sec:baseline}).
% Then, the MOVE algorithm is proposed to integrate the ideas of greedy and release algorithms (Section~\ref{sec:move}), which addresses their defects and combines the advantages.

\label{sec:onesource}
\vspace{1.5mm}
\noindent
\textbf{From Multiple Seeds to One Seed.}
For presentation simplicity, we introduce the techniques for the case of one seed vertex.
A unified seed vertex $s'$ is created to replace all the seeds in the graph. For each vertex $u$, if there are $h$ different seeds pointing to $u$ and the probability on each edge is $p_i (1\le i\le h)$, we remove all the edges from the seeds to $u$ and add an edge from $s'$ to $u$ with probability $(1-\prod_{i=1}^h (1-p_i))$. %We repeat the same operations on other vertices which are the out-neighbors of the sources. 
As an active vertex in the IC model only has one chance to activate every out-neighbor, the above modification will not affect the influence spread (i.e., expected spread in the graph) and the resulting blocker set is the same as the original problem.


\subsection{Baseline Algorithm}
\label{sec:baseline}

We first review and discuss the baseline greedy algorithm, which is the state-of-the-art for influence minimization (IMIN) problem and its variants \cite{min-greedy1,min-greedy-tree,min-greedy2,acycle-min-greedy,PhamPHPT19}. 

% \noindent \textbf{Greedy Algorithm.}
%Many previous works propose Greedy algorithm to solve the Influence Minimization Problem.
The greedy algorithm for the IC model is as follows: we start with an empty blocker set $B=\varnothing$, and then iteratively add vertex $u$ into set $B$ that leads to the largest decrease of expected spread, i.e., $u=\arg \max _{u\in V\setminus (S\cup B)}(\mathbb{E}(S,G[V\setminus B])-\mathbb{E}(S,G[V\setminus (B\cup \{u\})])$, until $|B|=b$.

Algorithm~A1 shows the details of the baseline greedy algorithm. The algorithm starts from an empty blocker set $B$ (Line 1). Then, in each iteration (Line 2), $x$ records the vertex whose blocking corresponds to the largest decrease of expected spread  (Line 3). The baseline greedy algorithm enumerates all the vertices to find the blocker with the maximum decrease of expected spread in each round (Lines 4-7) and insert it into the blocker set (Line 8). After $b$ iterations, the algorithm returns the blocker set $B$ (Line 9). 

\begin{algorithm}[t]
    \SetVline % save space
    \SetFuncSty{textsf}
    \SetArgSty{textsf}
	\caption{BaselineGreedy($G,s$)}
	\label{algo:greedy}
	\Input{a graph $G$ and the source $s$}
	\Output{the blocker set $B$}
	\State{$B\leftarrow $ empty}
	\For{$i\leftarrow 1$ to $b$}
	{
	    \State{$x\leftarrow -1$}
	    \For{each vertex in $u\in V(G)\setminus (B\cup \{s\})$}
	    {
	        \State{$\Delta [u]\leftarrow$ decrease of expected spread when blocking $u$}
	        \If{$x=-1$ or $\Delta [u] > \Delta[x]$}
	        {
	            \State{$x\leftarrow u$}
	        }
	    }
	    \State{$B\leftarrow B\cup \{x\}$}
	}
	\Return{$B$}
\end{algorithm}

As the previous works use Monte-Carlo Simulations to compute the expected spread for the greedy algorithm (Line 5 in Algorithm~A1), each computation of spread decrease needs $O(r\cdot m)$ time, where $r$ is the number of rounds in Monte-Carlo Simulations. Thus, the time complexity of Algorithm~A1 is $O(b\cdot n\cdot r\cdot m)$.

As indicated by the complexity, the baseline greedy algorithm cannot efficiently handle the cases with large $b$. 
The greedy heuristic is usually effective on small $b$ values, while the time cost is still large because it has to enumerate the whole vertex set as the candidate blockers and compute the expected spread for each candidate. % to find a blocker in each iteration.

% Previous works use Monte-Carlo Simulations to compute the expected spread for the greedy algorithm such that $T^{es}_{G}=r\cdot m$, where $r$ is the number of rounds of Monte-Carlo Simulations.
% We can see that Monte-Carlo Simulations lead to a huge computation cost.






\subsection{Efficient Algorithm for Candidate Selection}
\label{sec:candidates}

In this subsection, we propose an efficient algorithm for selecting the candidates.
We first show that the existing solutions for computing expected spread are infeasible to solve the IMIN problem efficiently (Section~\ref{sec:ec-exist}). Then, we propose a new framework (Section~\ref{sec:new-es}) based on sampled graphs (Section~\ref{sec::sample-graph}) and their dominator trees (Section~\ref{sec::domi-tree}) which can quickly compute the decrease of the expected spread of every candidate blocker through only one scan on the dominator trees.

\vspace{2.5mm}
\subsubsection{Existing Works}
\label{sec:ec-exist}

As computing the expected influence spread of a seed set in IC model is \#P-hard  \cite{maximization1}, and the exact solution can only be used in small graphs (e.g., with a few hundred edges) \cite{MaeharaSI17}. Thus, the existing works focus on estimation algorithms.
There are two directions as follows.


\vspace{2mm}
\noindent \textbf{Monte-Carlo Simulations (MCS).}
Kempe et al. \cite{first-max} apply Monte-Carlo Simulations to estimate the influence spread under IC model, which is often used in some influence related problems, e.g., \cite{OhsakaAYK14,MS-PCG,influencepath}. In each round of MCS, it removes every edge $(u,v)$ with $(1-p_{u,v})$ probability. Let $G'$ be the resulting graph, and the set $R(s)$ contains the vertices in $G'$ that are reachable from $s$ (i.e., there exists at least one path from $s$ to each vertex in $R(s)$). For the original graph $G$ and seed $s$, the expected size of set $R(s)$ equals to the expected spread $\mathbb{E}(\{s\},G)$ \cite{first-max}. 
%we can repeat multiple rounds to remove edges from $G$ to generate $G'$, and then calculate $R(s)$ on $G'$. The expected size (i.e., average size) of set $R(s)$ as an estimation of expected spread. 
Assuming we take $r$ rounds of MCS to estimate the expected spread, MCS needs $O(r\cdot m)$ times to calculate the expected spread. 
Recall that the influence minimization problem is to find the optimal blocker set with a given seed set.
The spread computation by MCS for influence minimization is costly, because the dynamic of influence spread caused by different blockers is not fully utilized in the sampling, and we have to repeatedly conduct MCS for each candidate blocker set.
%Note that the round number $r$ is set by user experience \cite{first-max} (e.g., $r=10000$) or an approximate function \cite{max-rr}.

\vspace{2mm}
\noindent \textbf{Reverse Influence Sampling (RIS).}
Borgs et al. \cite{Borgs-max} propose the Reverse Influence Sampling to approximately estimate the influence spread,  which is often used in the solutions for Influence Maximization (IMAX) problem, e.g., \cite{SunHYC18,Guo0WC20}. For each round, RIS generates an instance of $g$ randomly sampled from graph $G$ by removing each edge $(u,v)$ in $G$ with $(1-p_{u,v})$ probability, and then randomly sample a vertex $x$ in $g$. It performs reverse BFS to compute the reverse reachable (RR) set of the vertex $x$, i.e., the vertices which can be reached by vertex $x$ in the reverse graph of $g$. They prove that if the RR set of vertex $v$ has $\rho$ probability to contain the vertex $u$, when $u$ is the seed vertex, we have $\rho$ probability to activate $v$. 
In the IMAX problem, RIS generates RR sets by sampling the vertices in the sampled graphs and then applying the greedy heuristic. 
As the expected influence spread is submodular of seed set $S$ \cite{expectedspread}, an approximation ratio can be guaranteed by RIS in IMAX problem.
% However, we prove the expected spread is not submodular of blocker set $B$.
However, for our problem, reversing the graph is not helpful as the blockers seem ``intermediary" between the seeds and other vertices s.t. the computation cannot be unified into a single process in the reversing.
%However, it is not suitable for our problem. 
We prove the expected spread is not supermodular of blocker set $B$ which implies the absolute value of the marginal gain does not show a diminishing return.
Thus, the decrease of expected spread led by a blocker combination cannot be determined by the union effect of single blockers in the combination.


%But computing the expected spread through sampled graphs motivates us to propose the following algorithm for influence minimization problem.

% RIS degrades to MCS because different blocker combinations lead to different graph structures and the sampling should be re-conducted for each candidate blocker set.

\begin{figure*}[t]
\centering
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/sample-graph-1.pdf}
    \caption{Sampled graph 1}\label{fig:sample-example-a}
\end{subfigure}
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/sample-graph-2.pdf}
    \caption{Sampled graph 2}\label{fig:sample-example-b}
\end{subfigure}
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/sample-graph-3.pdf}
    \caption{Sampled graph 3}\label{fig:sample-example-c}
\end{subfigure}
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/sample-graph-4.pdf}
    \caption{Sampled Graph 4}\label{fig:sample-example-d}
\end{subfigure}
%\vspace{-1mm}
\caption{Sampled graphs of the graph $G$ in Figure~\ref{fig:sample}.}
\label{fig:sample-example}
\end{figure*}


\begin{figure*}[t]
\centering
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/dt-graph-1.pdf}
    \caption{DT of Sampled Graph 1}\label{fig:sample-dt-example-a}
\end{subfigure}
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/dt-graph-2.pdf}
    \caption{DT of Sampled Graph 2}\label{fig:sample-dt-example-b}
\end{subfigure}
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/dt-graph-3.pdf}
    \caption{DT of Sampled Graph 3}\label{fig:sample-dt-example-c}
\end{subfigure}
\begin{subfigure}[h]{0.205\linewidth}
    \includegraphics[width=1\columnwidth]{fig/dt-graph-4.pdf}
    \caption{DT of Sampled Graph 4}\label{fig:sample-dt-example-d}
\end{subfigure}
%\vspace{-1mm}
\caption{Dominator trees of sampled graphs in Figure~\ref{fig:sample-example}.}
\label{fig:sample-dt-example}
\end{figure*}

\vspace{2mm}
\subsubsection{Estimate the Expected Spread Decrease with Sampled Graphs} \label{sec::sample-graph}
We first define the random sampled graph.

\begin{definition}[Random Sampled Graph]
Let $\mathcal{G}$ be the distribution of the graphs with each induced by the randomness in edge removals from $G$, i.e., removing each edge $e=(u,v)$ in $G$ with $1-p_{u,v}$ probability. A random sampled graph $g$ derived from $G$ is an instance randomly sampled from $\mathcal{G}$.
\end{definition}

\begin{table}
    \caption{\revise{Summary of Notations for Random Sampled Graph}}
    \small
    \label{tab:nota-sampled}
       \centering
       \resizebox{\linewidth}{!}{
       \begin{tabular}{|p{0.15\columnwidth}|p{0.75\columnwidth}|}\hline
       \rowcolor[gray]{0.95} \revise{Notation} & \revise{Definition}\\ \hline\hline
       \revise{$\sigma(s,G)$} &
       \revise{the number of vertices reachable from $s$ in $G$}\\ \hline
       \revise{$\sigma^{\rightarrow u}(s,G)$} &
% \revise{the size of $\{v|(v\in V(G))\wedge(v$ can be reached from $s) \wedge ($all paths from $s$ to $v$ pass through $u)\}$}
\revise{the number of vertices reachable from $s$ in $G$, where all the paths from $s$ to these vertices pass through $u$}
       \\ \hline
%       \revise{$\sigma^{\not\rightarrow u}(s,G)$} & 
% % \revise{the size of $\{v|(v\in V(G))\wedge(v$ can be reached from $s) \wedge ($exist one path from $s$ to $v$ not pass through $u)\}$}
% \revise{the number of vertices reachable from $s$ in $G$ and all these vertices can be reached from $s$ without passing through $u$} 
%       \\ \hline
       \revise{$\xi^{\rightarrow u}(s,G)$} & \revise{the average number of $\sigma^{\rightarrow u}(s,G)$ in the sampled graphs which are derived from $G$}\\ \hline
       \end{tabular}}
\end{table}

\revise{We summarize the notations related to the random sampled graph in Table~\ref{tab:nota-sampled}.}
The following lemma is a useful interpretation of expected spread with IC model~\cite{MaeharaSI17}. 


\begin{lemma}
\label{lemma:sample}
Suppose that the graph $g$ is a random sampled graph derived from $G$. Let $s$ be a seed vertex, we have $\mathbb{E}[\sigma(s,g)]=\mathbb{E}(\{s\},G)$.
\end{lemma}

\revise{By Lemma~\ref{lemma:sample}, we have the following corollary for computing the expected spread when blocking one vertex.}


\begin{corollary}
\label{corollary::es-onevertex}
\revise{Given two fixed vertices $s$ and $u$ with $s\neq u$, and a random sampled graph $g$ derived from $G$, we have $\mathbb{E}[\sigma(s,g)-\sigma^{\rightarrow u}(s,g)]=\mathbb{E}(\{s\},G[V\setminus \{u\}])$.}
\end{corollary}

\begin{proof}
\revise{Let $g'=g[V(g)\setminus \{u\}]$, we have $\sigma(s,g)-\sigma^{\rightarrow u}(s,g)=\sigma(s,g')$. Thus, $\mathbb{E}[\sigma(s,g)-\sigma^{\rightarrow u}(s,g)]=\mathbb{E}[\sigma(s,g')]$. As $g'=g[V(g)\setminus \{u\}]$, $g'$ can be regarded as a random sampled graph derived from graph $G[V\setminus \{u\}]$. By Lemma~\ref{lemma:sample}, $\mathbb{E}[\sigma(s,g')]=\mathbb{E}(\{s\},G[V\setminus \{u\}])$. Therefore, $\mathbb{E}[\sigma(s,g)-\sigma^{\rightarrow u}(s,g)]=\mathbb{E}(\{s\},G[V\setminus \{u\}])$.}
\end{proof}


\revise{Based on Lemma~\ref{lemma:sample} and Corollary~\ref{corollary::es-onevertex}, we can compute the decrease of expected spread when a vertex is blocked.}



\begin{theorem}
Let $s$ be a fixed vertex, $u$ be a blocked vertex, and $g$ be a random sampled graph derived from $G$, respectively. For any vertex $u\in V(G)\setminus \{s\}$, we have the decrease of expected spread by blocking $u$ is equal to $\mathbb{E}[\sigma^{\rightarrow u}(s,g)]$, where $\mathbb{E}[\sigma^{\rightarrow u}(s,g)]=\mathbb{E}(\{s\},G)-\mathbb{E}(\{s\},G[V\setminus \{u\}])$.
\label{theo::block_expected}
\end{theorem}
% \vspace{-5mm}

\begin{proof}
% \sloppy
\revise{
As $\sigma^{\rightarrow u}(s,g)=\sigma(s,g)-(\sigma(s,g)-\sigma^{\rightarrow u}(s,g))$, we have $\mathbb{E}[\sigma^{\rightarrow u}(s,g)]=\mathbb{E}[\sigma(s,g)]-\mathbb{E}[\sigma(s,g)-\sigma^{\rightarrow u}(s,g)]$. 
From Corollary~\ref{corollary::es-onevertex}, we have $\mathbb{E}[\sigma(s,g)-\sigma^{\rightarrow u}(s,g)]=\mathbb{E}(\{s\},G[V\setminus \{u\}])$.
By Lemma~\ref{lemma:sample}, we know $\mathbb{E}[\sigma(s,g)]=\mathbb{E}(\{s\},G)$.
Therefore, $\mathbb{E}[\sigma^{\rightarrow u}(s,g)]=\mathbb{E}(\{s\},G)-\mathbb{E}(\{s\},G[V\setminus \{u\}])$.}
\end{proof}

As we use random sampling for estimating the decrease of expected spread of each vertex, we show that the average number of $\sigma^{\rightarrow u}(s,g)$ is an accurate estimator of any vertex $u$ and fixed seed vertex $s$, when the number of sampled graphs is sufficiently large. Let $\theta$ be the number of sampled graphs, $\xi^{\rightarrow u}(s,G)$ be the average number of $\sigma^{\rightarrow u}(s,g)$ and $OPT$ be the exact decrease of expected spread from blocking vertex $u$, i.e., $OPT=\mathbb{E}[\sigma^{\rightarrow u}(s,g)]$ (Theorem~\ref{theo::block_expected}). We use the Chernoff bounds~\cite{MotwaniR95} for theoretical analysis.

\begin{lemma}
Let $X$ be the sum of $c$ i.i.d. random variables sampled from a distribution on $[0,1]$ with a mean $\mu$. For any $\delta >0$, we have $Pr[X-c\mu \ge \delta \cdot c\mu] \le e^{-\delta^2c\mu /(2+\delta)}$ and $Pr[X-c\mu \le -\delta \cdot c\mu] \le e^{-\delta^2c\mu /2}.$
\label{lemma:cher}
\end{lemma}

\begin{theorem}
\label{theorem:approx}
For seed vertex $s$ and a fixed vertex $u$, the inequality $|\xi^{\rightarrow u}(s,G)-OPT| < \varepsilon\cdot OPT$ holds with at least $1-{n^{-l}}$ probability when $\theta\ge \frac{l(2+\varepsilon)n\log n}{\varepsilon^2\cdot OPT}$.
\end{theorem}

\begin{proof}
We have
$Pr[|\xi^{\rightarrow u}(s,G)-OPT|\ge \varepsilon\cdot OPT]$
$
\begin{matrix}
 =& Pr[|\frac{\xi^{\rightarrow u}(s,G)\cdot \theta}{n}-\frac{OPT\cdot \theta}{n}|\ge \frac{\varepsilon \cdot \theta}{n}\cdot OPT] \\
%=& Pr[|\frac{\xi^{\rightarrow u}(s,G)\cdot \theta}{n}-\mu \theta|\ge  \delta \cdot \theta \mu]
\end{matrix}
$.

Let $\delta=\varepsilon$, $\mu = \frac{OPT}{n}$ and $X=\frac{\xi^{\rightarrow u}(s,G)\cdot \theta}{n}$.
According to Lemma~\ref{lemma:cher}, we have
$Pr[|\xi^{\rightarrow u}(s,G)-OPT|\ge \varepsilon\cdot OPT]$
$=  Pr[|X-\theta \mu|\ge \delta \cdot \theta \mu] 
\le exp(\frac{-\delta^2\theta\mu}{2+\delta})
 = exp(\frac{-\varepsilon^2\theta OPT}{n(2+\varepsilon)})$.

% $
% \begin{matrix}
% = & Pr[|X-\theta \mu|\ge \delta \cdot \theta \mu] \\
%  \le & exp(\frac{-\delta^2\theta\mu}{2+\delta})\\
%  = & exp(\frac{-\varepsilon^2\theta OPT}{n(2+\varepsilon)})
% \end{matrix}
% $.

As $\theta\ge \frac{l(2+\varepsilon)n\log n}{\varepsilon^2\cdot OPT}$, we have $Pr[|\xi^{\rightarrow u}(s,G)-OPT|\ge \varepsilon\cdot OPT]\le exp(l \log n) = n^{-l}$.
Therefore, $|\xi^{\rightarrow u}(s,G)-OPT| < \varepsilon\cdot OPT$ holds with at least $1-n^{-l}$ probability.
\end{proof}




\subsubsection{Dominator Trees of Sampled Graphs}
\label{sec::domi-tree}

% \begin{algorithm}[t]
%     \SetVline % save space
%     \SetFuncSty{textsf}
%     \SetArgSty{textsf}
% 	\caption{Lengauer-Tarjan($G,s$)}
% 	\label{algo:lt}
% 	\Input{a graph $G$ and the source $s$}
% 	\Output{dominator tree $DT$}
% 	\State{Create a DFS tree $T$ through depth-first search}
% 	\State{Create a forest $F$ whose nodes set is $V(G)$ and does not contain any edges}
% 	\State{$B[\cdot]\leftarrow$ empty}
% 	\For{each $u\in V(G)\setminus \{s\}$ in reverse preorder by the DFS}
% 	{
%         \State{Compute $u$'s semidominator $sdom(u)$}
% 	    \State{Add $u$ into $B[sdom(u)]$}
% 	    \State{Add edge $(parent(u),u)$ into $F$}
% 	    \For{each $v\in B[parent(u)]$}
% 	    {
% 	        \If{$v$ is not the root in $F$}
% 	        {
% 	            \State{$r\leftarrow$ the root of the tree in $F$ which contains $v$}
% 	            \State{$w\leftarrow x\neq r$ of minimum $sdom(x)$ and on the path from $r$ to $v$ in $F$}
% 	        }
% 	        \Else{
% 	            \State{$w\leftarrow v$}
% 	        }
% 	        \If{$dfn(sdom(w)) < dfn(sdom(v))$}
% 	        {
% 	            \State{$idom(v)\leftarrow w$}
% 	        }
% 	        \Else{
% 	            \State{$idom(v)\leftarrow parent(u)$}
% 	        }
% 	    }
% 	    \State{$B[parent(u)]\leftarrow$ empty}
% 	}
% 	\For{each $u\in V(G)\setminus \{s\}$ in preorder by the DFS}
% 	{
% 	    \If{$idom(u)\neq sdom(u)$}
% 	    {
% 	        \State{$idom(u)\leftarrow idom(idom(u))$}
% 	    }
% 	    \State{Add edge $(idom(u),u)$ into $DT$}
% 	}
% 	\Return{$DT$}
% \end{algorithm}


In order to efficiently compute the decrease of expected spread when each vertex is blocked, we apply Lengauer-Tarjan algorithm to construct the dominator tree~\cite{LengauerT79}. 
Note that, in the following of this subsection, the id of each vertex is reassigned by the sequence of a DFS on the graph starting from the seed.

%Note that, in the following of this subsection, the id of a vertex is reassigned by the sequence of a DFS in the graph.
%To explain how it works, we first introduce the following concepts.

\begin{definition}[dominator]
Given $G=(V,E)$ and a source $s$, the vertex $u$ is a dominator of vertex $v$ when every path in $G$ from $s$ to $v$ has to go through $u$.
\end{definition}


\begin{definition}[immediate dominator]
Given $G=(V,E)$ and a source $s$, the vertex $u$ is the immediate dominator of vertex $v$, denoted $idom(v)=u$, if $u$ dominates $v$ and every other dominator of $v$ dominates $u$.
\end{definition}

We can find that every vertex except source $s$ has a unique immediate dominator. The dominator tree of graph $G$ is induced by the edge set $\{(idom(u),u)\mid u\in V\setminus \{s\}\}$ with root $s$ \cite{AhoU73,LowryM69}.

% \sloppy
Lengauer-Tarjan algorithm proposes an efficient algorithm for constructing the dominator tree.
It first computes the semidominator of each vertex $u$, denoted by $sdom(u)$, where $sdom(u)=\min \{v\mid \text{there is a path~} v=v_0,v_1,\cdots, v_k=u \text{~with~} v_i>u \text{~for any integer~} i\in [1, k)\}$. The semidominator can be computed by finding the minimum $sdom$ value on the paths of the DFS.
The core idea of Lengauer-Tarjan algorithm is to fast compute the immediate dominators by the semidominators based on the following lemma. The details of the algorithm can be found in~\cite{LengauerT79}.

\begin{lemma}~\cite{LengauerT79}
Given $G=(V,E)$ and a source $s$, let $u\neq s$ and $v$ be the vertex with the minimum $sdom(v)$ among the vertices in the paths from $sdom(u)$ to $u$ (including $u$ but excluding $sdom(u)$), then we have $$idom(u)=\left\{\begin{matrix}
sdom(u) & \text{if } sdom(u)=sdom(v), \\
idom(v) & \text{otherwise}. 
\end{matrix}\right.$$
\label{lemma:sdom2idom}
\vspace{-3mm}
\end{lemma}


% Algorithm~\ref{algo:lt} shows the pseudo-code of Lengauer-Tarjan algorithm.
% The algorithm first performs a depth-first search starting from vertex $s$ on the graph to build a DFS tree $T$ (Line 1), let $parent(u)$ denote the parent of vertex $u$ in $T$ and $dfn(u)$ denote the DFS number of vertex (i.e., numbering in order by reached during the DFS search). Then initialize the forest $F$ and $B[\cdot]$ (Line 2-3). For each vertex in reverse preorder by the DFS (Line 4), the algorithm first compute the semidominator and then use Lemma~\ref{lemma:sdom2idom} to compute the immediate dominator of each vertex (Line 6-21). Finally return the dominator tree by construct from edges $(idom(u),u)$ for each vertex $u$ (Line 22,23).

The time complexity of Lengauer-Tarjan algorithm is $O(m\cdot \alpha(m,n))$ which is almost linear, where $\alpha$ is the inverse function of Ackerman's function~\cite{ReelleZahlen}. 

\vspace{2mm}
\subsubsection{Compute the Expected Spread Decrease of Each Vertex}
\label{sec:new-es}
\revise{
Following the above subsections, if a vertex $u$ is blocked, we can use the number of vertices in the subtree rooted at $u$ in the dominator tree to estimate the decrease of expected spread. 
Thus, using a depth-first search of each dominator tree, we can accumulate the decrease of expected spread for every vertex if it is blocked.
}

\begin{algorithm}[t]
    \SetVline % save space
    \SetFuncSty{textsf}
    \SetArgSty{textsf}
	\caption{DecreaseESComputation($G,s,\theta$)}
	\label{algo:blockes}
	\Input{a graph $G$, the source $s$ and the number of sampled graphs $\theta$}
	\Output{$\Delta [u]$ for each $u\in V(G)\setminus \{s\}$, which is the decrease of expected spread when $u$ is blocked}
	\State{$\Delta[\cdot]\leftarrow 0$}
	\For{$i\leftarrow 1$ to $\theta$}
	{
	    \State{Generate a sampled graph $g$ derived from $G$}
    	\State{$DT\leftarrow$ the dominator tree of $g$ which is constructed by Lengauer-Tarjan algorithm~\cite{LengauerT79}}
    	\State{$c[\cdot]\leftarrow$ the size of subtree in tree $DT$ when each vertex is the root}
    	\For{each $u\in V(g)\setminus \{s\}$}
    	{
    	    $\Delta[u]\leftarrow \Delta[u] + c[u]/\theta$
    	}
	}

	\Return{$\Delta[\cdot]$}
\end{algorithm}



\begin{theorem}
\revise{Let $s$ be a fixed vertex in graph $g$. For any vertex $u\in (V(g)\setminus \{s\})$, we have $\sigma^{\rightarrow u}(s,g)$ equals to the size of the subtree rooted at $u$ in the dominator tree of graph $g$.}
\label{theo:dominator-subtree}
\end{theorem}

\begin{proof}
\revise{Let $c[u]$ denote the size of the subtree with root $u$ in the dominator tree of graph $g$. Assume $v$ is in the subtree with $u$ (i.e., $u$ is the ancestor of $v$), from the definition of dominator, we have $v$ cannot be reached by $s$ when $u$ is blocked. Thus, $c[u]\le \sigma^{\rightarrow u}(s,g)$. If $v$ is not in the subtree, i.e., $u$ does not dominate $v$ in the graph, there is a path from $s$ to $v$ not through $u$, which means blocking $u$ will not affect the reachability from $s$ to $v$. We have $\sigma^{\rightarrow u}(s,g) =  c[u]$.}
\end{proof}

Thus, for each blocker $u$, we can estimate the decrease of the expected spread by the average size of the subtrees rooted at $u$ in the dominator trees of the sampled graphs.


\begin{example}
Considering the graph $G$ in Figure~\ref{fig:sample}, there are only three edges with propagation probabilities less than $1$ (i.e., $(v_5,v_8)$, $(v_9,v_8)$ and $(v_8,v_7)$), and the other edges will exist in any sampled graph. 
Figures~\ref{fig:sample-example-a}-\ref{fig:sample-example-d} depict all the possible sampled graphs.
For conciseness, we use the dotted edge $(v_8,v_7)$ to represent whether it may exist in a sampled graph or not (corresponding to two different sampled graphs, respectively).
% Figure~\ref{fig:sample-example-a} shows a sampled graph contains $(v_5,v_8)$ and $(v_9,v_8)$, Figure~\ref{fig:sample-example-b} shows the sampled graph contains $(v_5,v_8)$, Figure~\ref{fig:sample-example-c} only contains $(v_9,v_8)$, and either $(v_5,v_8)$ or $(v_9,v_8)$ are not existed in Figure~\ref{fig:sample-example-d}. 
When $(v_8,v_7)$ is not in the sampled graphs, as $p_{v_5,v_8}=0.5$ and $p_{v_9,v_8}=0.2$, Figures~\ref{fig:sample-example-a}, \ref{fig:sample-example-b}, \ref{fig:sample-example-c} and \ref{fig:sample-example-d} have $0.1, 0.4, 0.1$ and $0.4$ to exist, respectively. 
As $p_{v_8,v_7}=0.1$, $v_1$ can reach $8+0.1=8.1$ vertices in expectation in Figure~\ref{fig:sample-example-a}. Similarly, $v_1$ can reach $8.1,8.1$ and $7$ vertices (including $v_1$) in expectation in Figures~\ref{fig:sample-example-b}, \ref{fig:sample-example-c} and  \ref{fig:sample-example-d}, respectively.
Thus, the expected spread of graph $G$ is $8.1\times (0.1+0.4+0.1)+7\times 0.4=7.66$, which is the same as the result we compute in Example~\ref{example:compute}.

Figures~\ref{fig:sample-dt-example-a}-\ref{fig:sample-dt-example-d} show the corresponding dominator trees of the sampled graphs in Figure~\ref{fig:sample-example}. For vertex $v_5$, the expected sizes of the subtrees rooted at $v_5$ are $5.1,5.1,5.1$ and $4$ in the dominator trees, respectively. Thus, the blocking of $v_5$ will lead to $5.1\times(0.1+0.4+0.1)+4\times 0.4=4.66$ decrease of expected spread. As the sizes of subtrees of $v_2,v_3,v_4$ and $v_6$ are only $1$ in each dominator tree, blocking any of them will lead to $1$ expected spread decrease. 
%As the expected size of $v_9$'s subtree is $1,1,2.1$ and $1$ in the dominator trees, respectively, blocking $v_9$ will lead to $1\times(0.1+0.4+0.4)+2.1\times 0.1=1.11$ decrease.
Similarly, blocking $v_7$, $v_8$ and $v_9$ will lead to $0.66$, $0.06$ and $1.11$ expected spread decrease, respectively.
\end{example}

Algorithm~\ref{algo:blockes} shows the details for computing the decrease of expected spread of each vertex. We set $\Delta[\cdot]$ as $0$ initially (Line 1). Then we generate $\theta$ different sampled graphs derived from $G$ (Lines 2-3). For each sampled graph, we first construct the dominator tree through Lengauer-Tarjan (Line 4). Then we use a simple DFS to compute the size of each subtree. After computing the average size of the subtrees and recording it in $\Delta[\cdot]$ (Lines 6-7), we return $\Delta[\cdot]$ (Line 8).

As computing the sizes of the subtrees through DFS costs $O(m)$, Algorithm~\ref{algo:blockes} runs in $O(\theta\cdot m\cdot \alpha(m,n))$.



\subsection{Our AdvancedGreedy Algorithm}
\label{sec:advanced-greedy}

\begin{algorithm}[t]
    \SetVline % save space
    \SetFuncSty{textsf}
    \SetArgSty{textsf}
	\caption{AdvancedGreedy($G,s,b,\theta$)}
	\label{algo:fast-greedy}
	\Input{a graph $G$, the source $s$, budget $b$ and the number of sampled graphs $\theta$}
	\Output{the blocker set $B$}
    \State{$B\leftarrow$ empty}
	\For{$i\leftarrow 1$ to $b$}
	{
	    \State{$\Delta[\cdot] \leftarrow$ DecreaseESComputation($G[V\setminus B],s,\theta$)}
	    \State{$x\leftarrow  -1$}
	    \For{each $u\in V(G)\setminus (\{S\}\cup B)$}
	    {
	        \If{$x=-1$ or $\Delta[u] > \Delta[x]$}
	        {
	            \State{$x\leftarrow u$}
	        }
	    }
	    \State{$B\leftarrow B\cup \{x\}$}
	}
	\Return{$B$}
\end{algorithm}

Based on Section~\ref{sec:baseline} and Section~\ref{sec:candidates}, we propose AdvancedGreedy algorithm with high efficiency.
In the greedy algorithm, we aim to greedily find the vertex $u$ that leads to the largest decrease of expected spread. Algorithm~\ref{algo:blockes} can efficiently compute the expected spread decrease of every candidate blocker.
Thus, we can directly choose the vertex which can cause the maximum decrease of expected spread (i.e., the maximum average size of the subtrees in the dominator trees derived from sampled graphs) as the blocker.

Algorithm~\ref{algo:fast-greedy} presents the pseudo-code of our AdvancedGreedy algorithm. We start with the empty blocker set (Line 1). In each of the $b$ iterations (Line 2), we first estimate the decrease of expected spread of each vertex (Line 3), find the vertex $x$ such that $\Delta[x]$ is the largest as the blocker (Lines 2-7) and insert it to blocker set (Line 8). Finally, the algorithm returns the blocker set $B$ (Line 9).

\vspace{1mm}
\noindent \textbf{Comparison with Baseline.}
one round of MCS on $G$ will generate a graph $G'$ where $V(G')=V(G)$ and each edge in $E(G)$ will appear in $G'$ if the simulation picks this edge.
% Thus the computation of expected spread through MCS and sampled graphs have the same effectiveness if $r=\theta$.
Thus, if we have $r=\theta$, our computation based on sampled graphs will not sacrifice the effectiveness, compared with MCS.
For efficiency, Algorithm~\ref{algo:fast-greedy} runs in $O(b\cdot \theta \cdot m\cdot \alpha(m,n) )$ and the time complexity of the saseline is $O(b\cdot r\cdot m\cdot n)$ (Algorithm~A1). As $\alpha(m,n)$ is much smaller than $n$, our AdvancedGreedy algorithm has a lower time complexity without sacrificing the effectiveness, compared with the baseline algorithm.

\subsection{The GreedyReplace Algorithm}
\label{sec:greedyreplace}

\revise{
Some out-neighbors of the seed may be an essential part of the result while they may be missed by current greedy heuristics. Thus, we propose a new heuristic (GreedyReplace) which is to first select $b$ out-neighbors of the seed as the initial blockers, and then greedily replace a blocker with another vertex if the expected spread will decrease.}


% We can find that if the budget is larger than or equal to the number of out-neighbors of the seed, we can choose to block all out-neighbors such that the influence spread is completely under control.
% %Besides, the greedy algorithm only considers selecting the optimal blocker in each round, which is not considering the cooperation between blockers. Motivated by this, we propose the GreedyReplace algorithm. From Theorem~\ref{theo:neighbor}, if the budget is relatively large or we want the expected spread of graph $G$ to be minimized, we must and only need to block all out-neighbors of seeds.
% However, the greedy algorithm chooses the vertex that leads to the largest decrease of expected spread each round, which may not be the out-neighbors of seeds. 
% Besides, only considering the out-neighbors of seeds as the candidate blockers may not be suitable when the budget is small.
% Thus we propose the GreedyReplace algorithm to combine these two methods.}


% \begin{theorem}
% For a fixed seed set $S$, if the expected spread of graph $G$ is minimized, i.e., expected spread of graph is $|S|$, all valid out-neighbors (i.e., the probability of the edges between seeds and their out-neighbors are larger than $0$) of seeds in $S$ must be blocked.
% \label{theo:neighbor}
% \end{theorem}

% \begin{proof}
% We prove it by contradiction. Suppose there is a valid out-neighbor $u$ which is not be blocked. As $u$ is the valid out-neighbor, there is a seed $s\in S$ satisfy that $p_{s,u} > 0$, thus the expected spread of graph must $\ge |S|+p_{s,u} > |S|$, which contradicts with expected spread $= |S|$.
% \end{proof}


\begin{example}
Considering the graph in Figure~\ref{fig:sample} with the seed $v_1$, Table~\ref{tab:motiv} shows the result of the Greedy algorithm and the result of only considering the out-neighbors as the candidate blockers (denoted as OutNeighbors). When $b=1$, Greedy chooses $v_5$ as the blocker because it leads to the largest expected spread decrease ($v_3,v_6,v_7,v_8$ and $v_9$ will not be influenced by $v_1$).
When $b = 2$, it further blocks $v_2$ or $v_4$ in the second round.
OutNeighbors only considers blocking $v_2$ and $v_4$. It blocks either of them when $b=1$, and blocks both of them when $b=2$.
\end{example}

% Based on this motivation, 

% \begin{algorithm}[t]
%     \SetVline % save space
%     \SetFuncSty{textsf}
%     \SetArgSty{textsf}
% 	\caption{GreedyNeighbor($G,s,b,\theta$)}
% 	\label{algo:greedy-neighbor}
% 	\Input{a graph $G$, the source $s$, budget $b$ and the number of sampled graphs $\theta$}
% 	\Output{the blocker set $B$}
%     \State{$CB\leftarrow N^{out}_s$}
%     \State{$B\leftarrow$ empty}
% 	\For{$i\leftarrow 1$ to $\min\{d^{out}_s,b\}$}
% 	{
% 	    \State{$\Delta[\cdot] \leftarrow$ DecreaseESComputation($G[V\setminus B],s,\theta$)}
% 	    \State{$x\leftarrow $ -1}
% 	    \For{each $u\in CB$}
% 	    {
% 	        \If{$x=-1$ or $\Delta[u] > \Delta[x]$}
% 	        {
% 	            \State{$x\leftarrow u$}
% 	        }
% 	    }
% 	    \State{$CB\leftarrow CB\setminus \{x\}$}
% 	    \State{$B\leftarrow B\cup \{x\}$}
% 	}
% 	\Return{$B$}
% \end{algorithm}

% \noindent \textbf{GreedyNeighbor Algorithm.}
% GreedyNeighbor algorithm is set all out-neighbors of seeds as the candidate blocker, and in each round, the algorithm choose one of the candidate blocker $u$ that leads to the largest decrease of expected spread.

% Algorithm~\ref{algo:greedy-neighbor} shows the details of GreedyNeighbor algorithm. We first push all out-neighbors of seed into candidate blocker set $CB$ (Line 1) and set blocker set empty initially (Line 2). For each round (Line 3), we choose the the candidate blocker which leads the largest expected spread decrease as the blocker (Line 4-8) and then update the $CB$ and $B$ (Line 9,10). Finally, the algorithm returns $B$ as the blocker set (Line 11).
% The time complexity of GreedyNeighbor is $O(\min \{d^{out}_s,b\}\cdot \theta \cdot m\alpha(m,n))$.

% \subsubsection{GreedyReplace Algorithm}

% \label{sec:move}

% \noindent \textbf{Motivations.}
% The following example illustrates the difference between the Greedy algorithm and the GreedyNeighbor algorithm.

% \begin{example}
% Considering the graph in Figure~\ref{fig:sample} with the seed $v_1$, Table~\ref{tab:motiv} shows the results of the Greedy algorithm and the GreedyNeighbor algorithm when $b=1$ and $b=2$. When $b=1$, Greedy chooses $v_5$ as the blocker because it can lead to largest expected spread decrease ($v_3,v_6,v_7,v_8$, and $v_9$ are inactive). When $b = 2$, it further blocks $v_2$ or $v_4$ in the second round. GreedyNeighbor algorithm only consider to block or release $v_2$ and $v_4$. It blocks either of them when $b=1$, and blocks both of them when $b=2$.
% \end{example}

\begin{table}[t]
\small
	\centering%
    %\vspace{-1mm}
	%\renewcommand{\arraystretch}{1.3}%
	\caption{Blockers and Their Expected Influence Spread}\label{tab:motiv}
	\resizebox{\linewidth}{!}{
	\begin{tabular}{c|c|c|c|c}
	\toprule
	\multirow{2}{*}{\centering Algorithm }& \multicolumn{2}{|c|}{$b=1$} & \multicolumn{2}{|c}{$b=2$}\\ \cline{2-5}
	 & $B$ & $\mathbb{E}(\cdot)$ & $B$ & $\mathbb{E}(\cdot)$ \\
	\midrule
	
	Greedy & $\{v_5\}$ & $3$ & $\{v_5,v_2$ or $v_4\}$ & $2$ \\ \hline
	OutNeighbors & $\{v_2$ or $v_4\}$ & $6.66$ &$\{v_2,v_4\}$ & $1$ \\ \hline
	GreedyReplace & $\{v_5\}$ & $3$ &$\{v_2,v_4\}$ & $1$ \\

	\bottomrule
	\end{tabular}
	}
% 	\vspace{2mm}
\end{table}

%If we use Greedy algorithm to choose the blockers, we will first choose $v_5$ as the blocker because it can lead to largest expected spread decrease (prevent $v_3,v_6,v_7,v_8,v_9$ from source). And then we will block $v_2$ and $v_4$. That is to say, if $\eta=0.5$, Greedy algorithm will just need to block one vertex $v_5$, but if $\eta=0$, Greedy algorithm have to block three vertices $v_2,v_4$ and $v_5$.

%Release algorithm will block $v_2,v_4$ and then consider releasing them, obviously, only block any one of them do not have any expected spread decrease. Thus, Release algorithm have to block $v_2$ and $v_4$ when $\eta=0$ or $\eta=0.5$.

In this example, we find that the performance of the Greedy algorithm is better than the OutNeighbors when $b$ is small, but its expected spread may become larger than OutNeighbors with the increase of $b$. 
% However, as in the time complexity, it is not efficient to use the Greedy Algorithm when $b$ is large.
% Besides, the Release algorithm may return an ineffective result given a small $b$ and a seed with many out-neighbors.
%This is also validated in our large scale experiments.
As the budget $b$ can be either small or large in different applications, it is essential to further improve the heuristic algorithm.


%The experiments show this law also holds true under normal circumstances.
%Besides, in the real application, to minimize the influence as much as possible, thus the budget may large. 



\begin{algorithm}[t]
    \SetVline % save space
    \SetFuncSty{textsf}
    \SetArgSty{textsf}
	\caption{GreedyReplace($G,s,b,\theta$)}
	\label{algo:greedyreplace}
	\Input{a graph $G$, the source $s$, budget $b$ and the number of sampled graphs $\theta$}
	\Output{the blocker set $B$}
	\State{$CB\leftarrow N^{out}_s$}
    \State{$B\leftarrow$ empty}
	\For{$i\leftarrow 1$ to $\min\{d^{out}_s,b\}$}
	{
	    \State{$\Delta[\cdot] \leftarrow$ DecreaseESComputation($G[V\setminus B],s,\theta$)}
	    \State{$x\leftarrow  -1$}
	    \For{each $u\in CB$}
	    {
	        \If{$x=-1$ or $\Delta[u] > \Delta[x]$}
	        {
	            \State{$x\leftarrow u$}
	        }
	    }
	    \State{$CB\leftarrow CB\setminus \{x\}$}
	    \State{$B\leftarrow B\cup \{x\}$}
	}
	
	\For{each $u\in B$ with the reversing order of insertion}
	{
	    \State{$B\leftarrow B\setminus \{u\}$}
	    \State{$\Delta[\cdot] \leftarrow$ DecreaseESComputation($G[V\setminus B],s,\theta$)}
	    \State{$x\leftarrow  -1$}
	    \For{each $u\in V(G)\setminus B$}
	    {
	        \If{$x=-1$ or $\Delta[u] > \Delta[x]$}
	        {
	            \State{$x\leftarrow u$}
	        }
	    }
	    \State{$B\leftarrow B\cup \{x\}$}
	    \If{$u=x$}
	    {
	        \State{Break}
	    }
	}
	\Return{$B$}
\end{algorithm}

% \noindent \textbf{GreedyReplace Algorithm.}


Due to the above motivation, based on Greedy and OutNeighbors, we propose the GreedyReplace algorithm to address their defects and combine the advantages.
We first greedily choose $b$ out-neighbors of the seed as the initial blockers. %In order to take advantage of the greedy heuristic, we consider greedily replacing a blocker with another vertex if the expected spread will decrease. Specifically, 
Then, we replace the blockers according to the reverse order of the out-neighbors' blocking order. %, e.g., we replace the vertex blocked in the latest round of OutNeighbors. 
As we can use Algorithm~\ref{algo:blockes} to compute the decrease of the expected spread of blocking any other vertex, in each round of replacement, we set all the vertices in $V(G)\setminus (\{s\}\cup B)$ as the candidates for replacement.
We will early terminate the replace procedure when the vertex to replace is current best blocker.

The expected spread of GreedyReplace is certainly not larger than the algorithm which only blocks the out-neighbors. Through the trade-off between choosing the out-neighbors and the replacement, the cooperation of the blockers is considered in GreedyReplace. % through which is not considered in the previous greedy algorithm. %The experiments show the Move method always has a better result than both Greedy and Release algorithms.

\begin{example}
\label{example:move}
Considering the graph in Figure~\ref{fig:sample} with the seed $v_1$, Table~\ref{tab:motiv} shows the results of three algorithms.
When $b=1$, GreedyReplace first consider the out-neighbors as the candidate blockers and set $v_2$ or $v_4$ as the blocker. As blocking $v_5$ can achieve smaller influence spread than both $v_2$ and $v_4$, it will replace the blocker with $v_5$. When $b=2$, GreedyReplace first block $v_2$ and $v_4$, and there is no better vertex to replace. The expected spread is $1$. GreedyReplace achieves the best performance for either $b=1$ or $b=2$.
%The results are shown in Table~\ref{tab:motiv}.
\end{example}


Algorithm~\ref{algo:greedyreplace} shows the pseudo-code of GreedyReplace. We first push all out-neighbors of the seed into candidate blocker set $CB$ (Line 1) and set blocker set empty initially (Line 2). For each round (Line 3), we choose the candidate blocker which leads to the largest expected spread decrease as the blocker (Lines 4-8) and then updates $CB$ and $B$ (Lines 9-10). 
% The time complexity of GreedyNeighbor is $O(\min \{d^{out}_s,b\}\cdot \theta \cdot m\alpha(m,n))$.
Then we consider replacing the blockers in $B$ by the reversing order of their insertions (Line 11). We remove the replaced vertex from the blocker set (Line 12) and use Algorithm~\ref{algo:blockes} to compute the decrease of expected spread $\Delta[\cdot]$ for each candidate blocker (Line 13).
We use $x$ to record the vertex with the largest spread decrease computed so far (Line 14), by enumerating each of the candidate blockers (Lines 15-17). 
%and update $x$ by $u$ if vertex $u$ is a better blocker
%After inserting the best blocker$x$ into the blocker set (Line 18), 
If the vertex to replace is current best blocker, we will early terminate the replacement (Lines 18-20). Algorithm~\ref{algo:greedyreplace} returns the set $B$ of $b$ blockers (Line 21).

The time complexity of GreedyReplace is $O(\min \{d^{out}_s,b\}\cdot \theta \cdot m\cdot \alpha(m,n))$. As the time complexity of Algorithm~\ref{algo:blockes} is mainly decided by the number of edges in the sampled graphs, thus in practice the time cost is much less than the worst case.
%MOVE algorithm can efficiently handle different scales of the budget $b$. 
%Greedy algorithm cannot handle small $b$ on moderate scale of graphs because it has to enumerate the vertex set and execute the spread computation for each vertex to find a blocker in each iteration. 
%As validated in the experiments, MOVE algorithm can efficiently handle different scales of budget $b$. %achieves a good trade-off between result quality and time cost, compared with Greedy and Release.

%We have $ T^{es}_{G}$ is much larger than $n$, thus the time complexity is $O((\max\{d^{out}_{s}-b,0\}\cdot d^{out}_{s}+m)\cdot T^{es}_{G})$. 

%In fact, it is difficult for Greedy algorithm to control the influence well (i.e., drastically decrease the expected spread) when $b$ is small, and it needs lots of time to computing if $b$ is large. However, our MOVE algorithm solves this awkward problem.


\subsection{\revise{Extension: IMIN Problem under Triggering Model}}

\revise{The triggering model is a generalization of both the IC model and the LT model~\cite{max-rr,first-max,Borgs-max}, which assumes that each vertex $u$ in $G$ is associated with a distribution $T(u)$ over subsets of $u$’s in-neighbors. 
For the given graph $G$, we can generate a sampled graph as follows: for each vertex $u$, we sample a triggering set of $u$ from $T(u)$, and remove each incoming edge of $u$ if the edge starts from a vertex not in the triggering set. With the sampled graphs, we can execute our AdvancedGreedy algorithm and GreedyReplace algorithm on them to solve the IMIN problem under the triggering model.}




% \subsection{Extension: Budget Minimization Problem}
% \label{sec:MBM}

% In real-life application, we sometimes want to find a set of blockers $B$ which has the minimum size such that the influence(i.e., expected spread) declines at least to the required threshold $\eta$ ratio of the initial influence. We define the formal problem below.


% \begin{definition}[\underline{B}udget \underline{M}inimization with \underline{D}eclining \underline{R}atio \underline{G}uarantee (BM-DRG) Problem]

% Given a directed social graph $G=(V,E)$, the influence probabilities $p_{u,v}$ on edges, a seed set $S$, a threshold $\eta \in [0,1]$. The Budget minimization with declining ratio guarantee (BM-DRG) problem aims to find the minimum size blocker set $B^*$ such that $\frac{\mathbb{E}(S,G[V\setminus B^*],V \setminus (S \cup B^*))}{\mathbb{E}(S,G,V\setminus (S \cup B^*))}\le \eta$, that is $$B^*={\arg \min} _{B:\frac{\mathbb{E}(S,G[V\setminus B],V\setminus (S \cup B))}{\mathbb{E}(S,G,V\setminus (S \cup B))}\le \eta} |B|$$.

% \end{definition}

% We first anlyze the hardness of the BM-DRG problem.

% For the BM-DRG problem, if $\eta=0$ we do not need to block any vertex, and when $\eta=1$, the optimal blocker set is all of the out-neighbors of the sources. However, the BM-DRG problem is NP-hard when $\eta\in (0,1)$, we will prove it by reducing the problem from the influence minimization problem.

% \begin{theorem}
% Given a graph $G$, if $\eta \in (0,1) $ the BM-DRG problem is NP-Hard.
% \label{theo::BM-DRGNP}
% \end{theorem}



% In addition, we prove the function is monotone of $\eta$.

% \begin{theorem}
% \label{theo:etamonotone}
% The function ${\arg \min} _{B:\frac{\mathbb{E}(S,G[V\setminus B],V\setminus (S \cup B))}{\mathbb{E}(S,G,V\setminus (S \cup B))}\le \eta} |B|$ is monotone of $\eta$.
% \end{theorem}



% We then extend our Move algorithm to Move based Budget Minimization (MBM) algorithm by using binary search to determine the minimal budget. The only problem for extension is how to calculate the minimal budgets for the given $\eta$. According to Theorem~\ref{theo:etamonotone}, we find that larger $\eta$ needs fewer budgets, thus we can use binary search to quickly get the minimal budget for the given $\eta$. Algorithm~\ref{algo:MBM} shows the pseudo-code for the MBM algorithm. \TODO{code  }

% The time complexity of Algorithm~\ref{algo:IP} is $O(\log_2(|\cup _{u\in S} N^{out}_u|) \cdot m\cdot T^{es}_{G})$, where $T^{es}_{G}$ is $O(n\cdot m)$ but much smaller than $nm$ in real graph, and we have $|\cup _{u\in S} N^{out}_u|\le n$.

% \begin{algorithm}[t]
%     \SetVline % save space
%     \SetFuncSty{textsf}
%     \SetArgSty{textsf}
% 	\caption{MBM($G,s,\eta$)}
% 	\label{algo:MBM}
% 	\Input{a graph $G$, the source $s$ and parameters $\eta$}
% 	\Output{the minimal budgets $b$}
% 	\State{$b_l=0,b_r=d^{out}_s$}
% 	\While{$b_l\le b_r$}
% 	{
% 	    \State{$b_{mid}=(l+r)/2$}
% 	    \State{$B\leftarrow Move(G,s,b_{mid})$}
%         \If{$\frac{\mathbb{E}(S,G[V\setminus B],V\setminus (S \cup B))}{\mathbb{E}(S,G,V\setminus (S \cup B))}\le \eta$}
%         {
%             \State{$b_r=b_{mid}-1$}
%         }
%         \Else{\State{$b_l=b_{mid}+1$}
%         }
% 	}
	
% 	\Return{$b=b_r+1$}
% \end{algorithm}


==> conclusion.tex <==
\section{Conclusion}


Minimizing the influence of misinformation is critical for a social network to serve as a reliable platform. 
In this paper, we systematically study the influence minimization problem to blocker $b$ vertices such that the influence spread of a given seed set is minimized. % for spread control of misinformation. %Given a graph $G$ and a budget $b$, the problem aims to find at most $b$ vertices in $G$ such that the blocking of these vertices leads to the largest decreasing influence spread on the graph. 
We prove the problem is NP-hard and hard to approximate.
A novel spread estimation algorithm is first proposed to largely improve the efficiency of state-of-the-art without sacrificing the effectiveness. Then we propose the GreedyReplace algorithm to refine the effectiveness of the greedy method by considering a new heuristic. % the cooperation between candidate blockers. % with a minor additional computation cost.
% The MOVE algorithm is proposed to combine the advantages of the greedy algorithms in previous works and our release algorithm. Besides, the IP algorithm is designed to quickly approach the exact result.
%in order to solve the problem of large time cost of computing expected spread in the graph, we propose the IP algorithm to quickly approach the exact result. 
Extensive experiments on 8 real-life datasets verify that our GreedyReplace and AdvancedGreedy algorithms largely outperform the competitors. % is more accurate and efficient than MCS, and MOVE will return the better result with less time than two baselines.
For future work, it is interesting to adapt our algorithm to other diffusion models and efficiently address other influence problems.
%We may also consider more factors, based on the fundamental influence minimization problem studied in this paper.



%In real-life applications, we sometimes want to find a minimal size of blocker set such that the influence(i.e., expected spread) declines at least to the required threshold ratio of the initial influence spread. As the expected spread of blocker size is monotone, our MOVE algorithm can easily extend to the budget minimization problem. Moreover, the proposed IP algorithm may inspire the computing for influence spread under other diffusion models (e.g., linear threshold model).

==> exp_MS.tex <==
\section{Experiments}
\label{sec:exp}

% In this section, extensive experiments are conducted to validate the effectiveness and efficiency of our proposed algorithms.

% \begin{figure}[!htbp]
%     \begin{minipage}{1\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/expected-spread-theta.pdf}
%     \caption{Expected Spread v.s. Number of Sampled Graphs}
%     \label{fig:es-theta}
%     \end{minipage}
%  \vspace{4mm}
        
%     \begin{minipage}{1\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-theta.pdf}
%     \caption{Running Time v.s. Number of Sampled Graphs}
%     \label{fig:time-theta}
%     \end{minipage}
%     \vspace{-1mm}
% \end{figure}

% \subsection{Experimental Setting}
% \label{sec:expset}

\noindent\textbf{Datasets.}
\jiadong{The experiments are conducted on $8$ real-world datasets, which are all publicly available from SNAP ({\url{http://snap.stanford.edu}}).
Table~\ref{tab:dat} shows the statistics of the datasets, ordered by the number of edges in each dataset, where $d_{avg}$ is the average node degree (the sum of in-degree and out-degree for each directed graph) and $d_{max}$ is the largest node degree.
For an undirected graph, we consider each edge as bi-directional. These experiments cover a diverse range of networks, spanning from networks consisting of 1,000 nodes and 25,000 edges to networks comprising 1 million nodes and 3 million edges.}
% {\color{red} TODO: for each dataset, describe (1) what is this dataset about (e.g., DBLP is computer science bibliography database), (2) what does node represent (3) what does edge represent }




\noindent \textbf{Propagation Models.} 
Our algorithm is designed for the IC and LT models with nonuniform propagation probabilities $p_{u,v}$ for each directed edge $(u,v)$. To generate these nonuniform probabilities $p_{u,v}$, we employ two propagation models following the existing literature:% \citep[e.g.,][]{first-max,maximization1}.
% \begin{enumerate}
(i). Trivalency (TR) model \citep{JungHC12,maximization1,min-greedy-tree}: The propagation probability $p_{u,v}$ for each edge $(u,v)$ is randomly chosen from the set \{0.1, 0.01, 0.001\}, which correspond to high, medium, and low influences, respectively.
(ii). Weighted cascade (WC) model \citep{first-max,max-rr}: The propagation probability $p_{u,v}$ for each edge $(u,v)$ is $1/d^{in}_v$, where $d^{in}_v$ is the in-degree of $v$.
% \end{enumerate}

\vspace{-3mm}
\begin{table}[!htbp]\color{jiadong}
	\caption{\jiadong{Statistics of Datasets}}
	\centering%
	\renewcommand{\arraystretch}{1.3}%
	\resizebox{\linewidth}{!}{
	\begin{tabular}{|lc|lcl|ccccc|}
	\toprule
	\bf{Dataset} & Abbr. & Description & Node & Edge $(u,v)$ & \bf{$n$} & \bf{$m$} & \bf{$d_{avg}$} & \bf{$d_{max}$} & \bf{Type}  \\
		\midrule
		EmailCore & EC & email data& member & $u$ sent at least one email to $v$ & 1,005 & 25,571 &  49.6 &544 & Directed\\
		Facebook & F & social network & user & $u$ and $v$ are friends & 4,039 & 88,234 & 43.7 & 1,045  & Undirected \\
		Wiki-Vote & W &vote data & user &  $u$ voted on user $v$  & 7,115 & 103,689 & 29.1 & 1,167 & Directed\\
		
		
		EmailAll & EA& email data& user & $u$ sent at least one email to $v$  & 265,214 & 420,045 & 3.2 & 7,636 & Directed\\
		DBLP & D&bibliography & author & $u$ and $v$ are co-authors & 317,080 & 1,049,866 & 6.6 & 343 & Undirected\\
		
		Twitter & T &social network & user & $u$ and $v$ are friends & 81,306 & 1,768,149 & 59.5& 10,336  & Directed\\
		
		Stanford & S & website pages & page & $u$ has hyperlinks to $v$ & 281,903 & 2,312,497 & 16.4 & 38,626 & Directed\\
		Youtube & Y&social network & user & $u$ and $v$ are friends  & 1,134,890 & 2,987,624 & 5.3 & 28,754 & Undirected\\
		
		\bottomrule
	\end{tabular}
	}
	\label{tab:dat}
\end{table}



\noindent \textbf{Settings.}
Unless otherwise specified, we set $r=10^4$ for MCS
% {\color{red} This is not $10^5$ as you commented below}
, and for our sampled-graph-based algorithms (AdvancedGreedy and GreedyReplace), we sample $10^4$ graphs in the experiments. In each of our experiments, we independently execute each algorithm 5 times and report the average result. By default, we terminate an algorithm if the running time reaches 24 hours.
% Note that all expected spread are computed by Monte-Carlo Simulations with $10^5$ rounds. %To make the experimental results more objective and fair
Based on the results of the $\theta$ selection study (details in the online appendix 4), we set $\theta=10^4$ for all experiments.

\noindent \textbf{Environments.} The experiments are performed on a CentOS Linux server (Release 7.5.1804) with Quad-Core Intel Xeon CPU (E5-2640 v4 @ 2.20GHz) and 128G memory. All the algorithms are implemented in C++. The source code is compiled by GCC(7.3.0) under O3 optimization.

\noindent \textbf{Algorithms.}
The experiments involve comparing our proposed algorithms, namely the GreedyReplace and AdvancedGreedy, with both the greedy algorithms and other basic heuristics mentioned in the existing literature. The algorithms evaluated in our experiments are listed below.
% \begin{enumerate}

\noindent 1. \underline{\texttt{Exact}}
% \citep{MaeharaSI17} {\color{red} is the reference correct?}
: This algorithm identifies the optimal solution by searching all possible combinations of $b$ blockers and uses MCS with $r=10^4$ to compute the expected spread of candidate set of blockers. The algorithms show optimal effectiveness without considering efficiency, providing a benchmark for effectiveness comparison.

\noindent 2. \underline{\texttt{Rand} (RA)}: This algorithm randomly chooses $b$ blockers (excluding the seeds) in the graph.

\noindent 3. \underline{\texttt{OutDegree} (OD)} \citep{Nature-error,Viruses}: This algorithm selects $b$ nodes with the highest out-degrees as the blockers for the IMIN problem and selects $b$ directed edges where the ending nodes have the highest out-degrees {for IMIN-EB problem}.
% \noindent \underline{\texttt{SPIN} (SP)}: Shapely value-based approach algorithm SPIN. It is proposed to solve the $\lambda$-Coverage Problem\cite{max-ratio}, but it can also used for BM-DRG problem. The algorithm select the nodes as the blockers according to descending order of Shapley value, i.e., $\Phi(N,i)=\sum _{C\subseteq N\setminus \{i\}} \frac{|C|!(n-|C|-1)!}{n!} (va(C\cup \{i\})-va(C))$ where $N=V\setminus S$ and $va$ is the value of expected spread.
% \noindent \underline{\texttt{Monte-Carlo Simulations} (MCS)}: The existing algorithm for estimating the expected spread (Section~\ref{sec:ec-exist}) \cite{first-max}.

{\noindent 4. \underline{\texttt{GRASP} (GS)} \citep{FeoR95}: Greedy Randomized Adaptive Search (GRASP) is a metaheuristic algorithm commonly utilized for combinatorial optimization problems. It involves iterations comprising the sequential construction of a greedy randomized solution followed by iterative enhancements through local search. We run it one iteration since it needs a large time cost.}

\noindent 5. \underline{\texttt{BaselineGreedy} (BG)} \citep{min-greedy2,min-greedy1,min-greedy-tree}: This algorithm represents the current state-of-the-art approach. We have introduced and discussed in detail in Section \ref{sec:baseline}. It leverages the MCS technique to estimate the expected spread.



\noindent 6. \underline{\texttt{AdvancedGreedy} (AG)}: Our proposed AdvancedGreedy algorithm (Algorithm~\ref{algo:fast-greedy}), which applies dominator tree techniques for estimating the reduction of expected spread.

\noindent 7. \underline{\texttt{GreedyReplace} (GR)}: Our proposed GreedyReplace algorithm (Algorithm~\ref{algo:greedyreplace}). It enhances the AdvancedGreedy algorithm by considering the relationships among candidate blockers.
% \end{enumerate}

{\noindent \textbf{Availability.}
The datasets, source code, and detailed results are available online~\citep{IM2024}.}

% Our source code is shared online\footnote{\url{https://www.dropbox.com/sh/k8w65cgr2ka68r9/AAAQGzqn3DgukWOcoQAYzxRta?dl=0}}. 

% \subsection{Study of $\theta$ Selection}

% In this section, we provide the justification for selecting $\theta$ (i.e., the number of sampled graphs), which represents the number of sampled graphs used to choose the blocker in each round. 

% % \noindent {\bf Varying the Number of Sampled Graphs.}
% % {\color{red} Should this part be put outside of this Effectiveness Comparison Section? This one is not relevant for effectiveness.}
% In Figure~\ref{fig:es-theta} and Figure~\ref{fig:time-theta}, we vary $\theta$ from $10^3$, $10^4$ to $10^5$, and report the expected spread and running time of our GR algorithm. 
% %Note that the base value of the expected spread is computed by Monte-Carlo Simulations with $10^5$ rounds, and we check the margins.
% We evaluate on all datasets under the TR model by setting the blocker budget to $20$ and randomly selecting $10$ seed nodes. The y-axis is the decrease ratio of the expected spread\footnote{We show the decrease ratio because the absolute differences of expected spreads are quite small.} using three $\theta$ values in Figure~\ref{fig:es-theta} and the running time (s) in Figure~\ref{fig:time-theta}. The x-axis represents different networks whose abbreviations are listed in Table \ref{tab:dat} column (2).
% From Figure ~\ref{fig:es-theta}, we observe that the largest decrease ratio from $\theta=10^3$ to $\theta=10^4$ is only $2.89\%$, and the largest decrease ratio from $\theta=10^4$ to $\theta=10^5$ is less than $0.1\%$.
% Figure~\ref{fig:time-theta} shows the running time gradually increases when $\theta$ increases. 
% Based on the obtained results, we selected a value of $\theta=10^4$ for all experiments, as it provided a favorable balance between time costs and accuracy. %related to the scale of the graph, and will

% % \begin{figure}[!htbp]
% %     \centering
% %     \includegraphics[width=0.7\linewidth]{fig/expected-spread-theta.pdf}
% %     \caption{Expected Spread v.s. Number of Sampled Graphs}
% %     \label{fig:es-theta}
% % \end{figure}

% % \begin{figure}[!htbp]
% %     \centering
% %     \includegraphics[width=0.7\linewidth]{fig/time-theta.pdf}
% %     \caption{Running Time v.s. Number of Sampled Graphs}
% %     \label{fig:time-theta}
% % \end{figure}

% \begin{figure}[!htbp]
% \begin{subfigure}[h]{0.47\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/expected-spread-theta.pdf}
%     \caption{Expected Spread v.s. \#Sampled Graphs}
%     \label{fig:es-theta}
%     \end{subfigure}
% \begin{subfigure}[h]{0.47\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-theta.pdf}
%     \caption{Running Time v.s. Number of Sampled Graphs}
%     \label{fig:time-theta}
%     \end{subfigure}
%     \caption{Time Cost of Different Algorithms} \label{fig:time}
% \end{figure}


% \subsection{Effectiveness Comparison}
% In this section, we first evaluate our proposed algorithms in comparison to the Exact algorithm, which represents the maximum achievable effectiveness without considering efficiency. Then we evaluate the efficacy of our proposed algorithms in comparison to other existing heuristics documented in the literature.

\noindent \textbf{Comparison with the Exact Algorithm.}
\jiadong{As AG has an approximate guarantee under the LT model in both IMIN problem and IMIN-EB problem, we only compare the result of GR with the \texttt{Exact} algorithm under the IC model in two problems.
% The comparison results under the WC model are shown in Table A2 in online appendix.
Due to the huge time cost of \texttt{Exact}, we extract small datasets by iteratively extracting a node and all its neighbors, until the number of extracted nodes reaches $100$ in IMIN problem (resp. edges reaches $100$ in IMIN-EB problem). 
% For \texttt{EmailCore} under both WC and TR models, we extract $5$ such subgraphs.
For \texttt{EmailCore}, we extract $5$ such subgraphs.
We randomly choose $10$ nodes as the seeds. As the graph is small, we can use the exact computation of the expected spread~\citep{MaeharaSI17} for comparison between \texttt{Exact} and GR.
We demonstrate that the expected spread of the GR algorithm closely aligns with the results of the Exact algorithm in both the TR Model (Tables~\ref{tab:exact} Panel A and Panel B) and the WC Model (Table A2 Panel C and Panel D in online appendix). Additionally, the GR algorithm outperforms the Exact algorithm in terms of speed, with a difference of up to six orders of magnitude in both the IMIN problem and the IMIN-EB problem. The results indicate that our proposed algorithms are highly effective and can achieve optimal results in a shorter timeframe.}


\begin{table}[!htbp]\color{jiadong}
    \centering
\caption{Exact v.s. GreedyReplace (IC model)}\label{tab:exact}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
\multirow{2}{*}{ b } & \multicolumn{3}{c|}{Expected Spread} & \multicolumn{2}{c|}{Running Time (s)} & \multicolumn{3}{c|}{Expected Spread} & \multicolumn{2}{c|}{Running Time (s)}  \\ \cline{2-11}
& Exact & GR & Ratio & Exact & GR & Exact & GR & Ratio & Exact & GR \\ 
\midrule
& \multicolumn{5}{c|}{Panel A: IMIN Problem (TR Model)} & \multicolumn{5}{c|}{Panel B: IMIN-EB Problem (TR Model)}\\
\midrule
1 & 12.614 & 12.614 & 100\% & 3.07 & 0.12 & 10.873 & 10.873 & 100\% & 3.04 & 0.10 \\
2 & 12.328 & 12.334 & 99.95\% & 130.91 & 0.21 & 10.652 & 10.655 & 99.9\% & 150.72 & 0.31 \\
3 & 12.112 & 12.119 & 99.94\% & 3828.2 & 0.25 & 10.454 & 10.459 & 99.9\% & 5373.9 & 0.35 \\
4 & 11.889 & 11.903 & 99.88\% & 80050 & 0.33 & 10.360 & 10.407 & 99.5\% & 90897 & 0.40 \\ 
\midrule
% \multicolumn{6}{l}{Panel B: IMIN Problem (WC Model)}\\
% \midrule
% 1 & 11.185 & 11.185 & 100\% & 2.63 & 0.10 \\
% 2 & 11.077 & 11.078 & 99.99\% & 110.92 & 0.18 \\
% 3 & 10.997 & 10.998 & 99.99\% & 3284.0 & 0.23 \\
% 4 & 10.922 & 10.925 & 99.97\% & 69415 & 0.33 \\ 
% \midrule
% & \multicolumn{5}{c|}{Panel C: IMIN-EB Problem (TR Model)} &\multicolumn{5}{c|}{Panel D: IMIN-EB Problem (WC Model)}\\
% \midrule
% 1 & 10.873 & 10.873 & 100\% & 3.04 & 0.10 & 11.882 & 11.882 & 100\% & 4.03 & 0.12 \\
% 2 & 10.652 & 10.655 & 99.9\% & 150.72 & 0.31 & 11.634 & 11.697 & 99.5\% & 205.21 & 0.25  \\
% 3 & 10.454 & 10.459 & 99.9\% & 5373.9 & 0.35 & 11.344 & 11.421 & 99.3\% & 7375.2 & 0.37  \\
% 4 & 10.360 & 10.407 & 99.5\% & 90897 & 0.40 & 11.269 & 11.279 & 99.9\% & 98247 & 0.50 \\
% \midrule
% \multicolumn{6}{l}{Panel D: IMIN-EB Problem (WC Model)}\\
% \midrule
% 1 & 11.882 & 11.882 & 100\% & 4.03 & 0.12 \\
% 2 & 11.634 & 11.697 & 99.5\% & 205.21 & 0.25 \\
% 3 & 11.344 & 11.421 & 99.3\% & 7375.2 & 0.37  \\
% 4 & 11.269 & 11.279 & 99.9\% & 98247 & 0.50 \\
\bottomrule
\end{tabular}
}
\vspace{-5mm}
\end{table}


% \begin{table}[!htbp]
%     \centering
% \caption{Exact v.s. GreedyReplace}\label{tab:exact}
% % \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
% \toprule
% \multirow{2}{*}{ b } & \multicolumn{3}{c|}{Expected Spread} & \multicolumn{2}{c|}{Running Time (s)} & \multicolumn{3}{c|}{Expected Spread} & \multicolumn{2}{c|}{Running Time (s)}  \\ \cline{2-11}
% & Exact & GR & Ratio & Exact & GR & Exact & GR & Ratio & Exact & GR \\ 
% \midrule
% & \multicolumn{5}{c|}{Panel A: IMIN Problem (TR Model)} & \multicolumn{5}{c|}{Panel B: IMIN Problem (WC Model)}\\
% \midrule
% 1 & 12.614 & 12.614 & 100\% & 3.07 & 0.12 & 11.185 & 11.185 & 100\% & 2.63 & 0.10 \\
% 2 & 12.328 & 12.334 & 99.95\% & 130.91 & 0.21 & 11.077 & 11.078 & 99.99\% & 110.92 & 0.18 \\
% 3 & 12.112 & 12.119 & 99.94\% & 3828.2 & 0.25 & 10.997 & 10.998 & 99.99\% & 3284.0 & 0.23 \\
% 4 & 11.889 & 11.903 & 99.88\% & 80050 & 0.33 & 10.922 & 10.925 & 99.97\% & 69415 & 0.33 \\ 
% \midrule
% % \multicolumn{6}{l}{Panel B: IMIN Problem (WC Model)}\\
% % \midrule
% % 1 & 11.185 & 11.185 & 100\% & 2.63 & 0.10 \\
% % 2 & 11.077 & 11.078 & 99.99\% & 110.92 & 0.18 \\
% % 3 & 10.997 & 10.998 & 99.99\% & 3284.0 & 0.23 \\
% % 4 & 10.922 & 10.925 & 99.97\% & 69415 & 0.33 \\ 
% % \midrule
% & \multicolumn{5}{c|}{Panel C: IMIN-EB Problem (TR Model)} &\multicolumn{5}{c|}{Panel D: IMIN-EB Problem (WC Model)}\\
% \midrule
% 1 & 10.873 & 10.873 & 100\% & 3.04 & 0.10 & 11.882 & 11.882 & 100\% & 4.03 & 0.12 \\
% 2 & 10.652 & 10.655 & 99.9\% & 150.72 & 0.31 & 11.634 & 11.697 & 99.5\% & 205.21 & 0.25  \\
% 3 & 10.454 & 10.459 & 99.9\% & 5373.9 & 0.35 & 11.344 & 11.421 & 99.3\% & 7375.2 & 0.37  \\
% 4 & 10.360 & 10.407 & 99.5\% & 90897 & 0.40 & 11.269 & 11.279 & 99.9\% & 98247 & 0.50 \\
% % \midrule
% % \multicolumn{6}{l}{Panel D: IMIN-EB Problem (WC Model)}\\
% % \midrule
% % 1 & 11.882 & 11.882 & 100\% & 4.03 & 0.12 \\
% % 2 & 11.634 & 11.697 & 99.5\% & 205.21 & 0.25 \\
% % 3 & 11.344 & 11.421 & 99.3\% & 7375.2 & 0.37  \\
% % 4 & 11.269 & 11.279 & 99.9\% & 98247 & 0.50 \\
% \bottomrule
% \end{tabular}
% % }
% \end{table}






% \noindent \textbf{Characteristics of Blocker Set.}
% \TODO{ if needs}





%\subsection{}





% \vspace{-8mm}
\begin{table*}[!htbp]
\centering
\caption{Expected Spread in the IMIN problem (IC model)}\label{table:heuristics}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|lllll|lllll|lllll|lllll}
\toprule
\multirow{2}{*}{\centering b } & \multicolumn{5}{c|}{EmailCore (TR model)} & \multicolumn{5}{c|}{Facebook (TR model)} & \multicolumn{5}{c|}{Wiki-Vote (TR model)} & \multicolumn{5}{c}{EmailAll (TR model)} \\
& RA & OD & GS & AG & GR & RA & OD & GS & AG & GR & RA & OD & GS & AG & GR & RA & OD & GS & AG & GR \\
\midrule
20 & 354.88$^{***}$ & 230.10$^{***}$ & 223.45$^{**}$ & 220.59$^{**}$ & \bf{219.69}
& 16.059$^{***}$ & 16.026$^{***}$&12.134$^{**}$ & 11.717$^{*}$ & \bf{11.691}
& 512.62$^{***}$ & 325.51$^{***}$&135.935$^{***}$ & 131.30$^{*}$ & \bf{130.77}
& 548.99$^{***}$ & 286.05$^{***}$ &14.925$^{***}$& 14.642$^{**}$ & \bf{13.640} \\
40 & 341.33$^{***}$ & 98.712$^{***}$ &85.193$^{***}$& 84.022$^{*}$ & \bf{83.823}
& 16.037$^{***}$ & 16.019$^{***}$ &10.509$^{*}$ & 10.416$^{*}$ & \bf{10.413}
& 512.18$^{***}$ & 222.00$^{***}$ &45.931$^{***}$ & 46.747$^{***}$ & \bf{43.898}
& 546.94$^{***}$ & 221.97$^{***}$ &10.310$^{*}$ & 10.319$^{*}$ & \bf{10.002} \\
60 & 325.13$^{***}$ & 47.249$^{***}$ & 35.092$^{**}$ & 35.085$^{**}$ & \bf{33.634}
& 16.033$^{***}$ & 16.010$^{***}$ &10.151$^{*}$& 10.151$^{*}$ & \bf{10.149}
& 507.11$^{***}$ & 138.60$^{***}$ &25.013$^{***}$ & 25.514$^{***}$ & \bf{23.282}
& 546.39$^{***}$ & 148.52$^{***}$ &10.003$^{*}$& 10 & 10 \\
80 & 304.90$^{***}$ & 30.277$^{***}$ &18.996$^{*}$ & 19.001$^{*}$ & \bf{18.848}
& 15.997$^{***}$ & 15.987$^{***}$ &10.031$^{*}$& 10.028$^{*}$ & \bf{10.026}
& 501.49$^{***}$ & 32.646$^{***}$ &17.398$^{*}$ & 17.332$^{*}$ & \bf{17.322}
& 545.41$^{***}$ & 100.84$^{***}$ &10& 10 & 10 \\
100 & 283.54$^{***}$ & 22.696$^{***}$ &13.595$^{*}$ & 13.640$^{*}$
& \bf{13.533} & 15.994$^{***}$ & 15.980$^{***}$&10.003$^{*}$ & 10.001 & 10.001
& 496.05$^{***}$ & 25.831$^{***}$ &14.720$^{*}$ & 14.726$^{*}$ & \bf{14.518}
& 544.59$^{***}$ & 55.398$^{***}$ &10& 10 & 10 \\
\bottomrule

\toprule
\multirow{2}{*}{\centering b } & \multicolumn{5}{c|}{DBLP (TR model)} & \multicolumn{5}{c|}{Twitter (TR model)} & \multicolumn{5}{c|}{Stanford (TR model)} & \multicolumn{5}{c}{Youtube (TR model)} \\
& RA & OD & GS & AG & GR & RA & OD & GS & AG & GR & RA & OD & GS & AG & GR & RA & OD & GS & AG & GR \\
\midrule
20 & 13.747$^{***}$ & 13.730$^{***}$ & 10.508$^{*}$& 10.502$^{*}$ & \bf{10.499}
& 16,801$^{***}$ & 16,610$^{***}$ & 16,103$^{**}$ &16,101$^{*}$ & \bf{16,100}
& 16.087$^{***}$ & 16.075$^{***}$ & 11.872$^{***}$ &12.069$^{***}$ & \bf{10.483}
& 14.774$^{***}$ & 14.762$^{***}$ &13.431$^{***}$ & 14.743$^{***}$ & \bf{10.950} \\

40 & 13.739$^{***}$ & 13.725$^{***}$ & 10.084$^{*}$& 10.079 & 10.079
& 16,796$^{***}$ & 16,470$^{***}$ & 15,749$^{**}$ & 15,749$^{**}$ & \bf{15,748}
& 16.080$^{***}$ & 16.071$^{***}$ & 10.493$^{*}$ & 10.488$^{*}$ & \bf{10.234}
& 14.773$^{***}$ & 14.755$^{***}$ & 10.009$^{*}$ &10.075$^{*}$ & \bf{10.002} \\

60 & 13.737$^{***}$ & 13.721$^{***}$ & 10.014$^{*}$& 10.012$^{*}$ & \bf{10.010}
& 16,786$^{***}$ & 16,329$^{***}$ & 15,015$^{***}$ &15,447$^{***}$ & \bf{14,972}
& 16.071$^{***}$ & 16.040$^{***}$ & 10.115$^{*}$ & 10.136$^{*}$ & \bf{10.075}
& 14.773$^{***}$ & 14.750$^{***}$ & 10& 10 & 10 \\

80 & 13.720$^{***}$ & 13.714$^{***}$ & 10 & 10 & 10
& 16,780$^{***}$ & 16,175$^{***}$ & 14,524$^{***}$ &14,610$^{***}$ & \bf{14,474}
& 16.064$^{***}$ & 16.017$^{***}$ & 10.022$^{*}$ &10.026$^{*}$ & \bf{10.019}
& 14.767$^{***}$ & 14.742$^{***}$ & 10& 10 & 10 \\

100 & 13.716$^{***}$ & 13.706$^{***}$& 10  & 10 & 10 &
16,771$^{***}$ & 16,057$^{***}$ & 13,439$^{***}$ &13,619$^{***}$ & \bf{13,181}
& 16.052$^{***}$ & 15.989$^{***}$ & 10.008$^{*}$ &10.009$^{*}$ & \bf{10.002}
& 14.762$^{***}$ & 14.729$^{***}$ & 10& 10 & 10 \\
\bottomrule

\multicolumn{13}{l}{\begin{minipage}{1.1\textwidth}  Notes. Best performers are bold. All experiments are repeated five times.

~~~~~~~~~~~~~~$^{*}p<0.1$; $^{**}p<0.05$; $^{***}p<0.001$.
\end{minipage}}

% \toprule
% \multirow{2}{*}{\centering b } & \multicolumn{4}{c|}{EmailCore (WC model)} & \multicolumn{4}{c|}{Facebook (WC model)} & \multicolumn{4}{c|}{Wiki-Vote (WC model)} & \multicolumn{4}{c}{EmailAll (WC model)} \\
% & RA & OD & AG & GR & RA & OD & AG & GR & RA & OD & AG & GR & RA & OD & AG & GR \\
% \midrule
% 20 & 82.605 & 54.907 & 53.516 & \bf{53.296} & 21.482 & 21.362 & 14.588 & \bf{14.554} & 24.102 & 22.660 & 17.765 & \bf{17.701} & 13.330 & 11.493 & 10.720 & \bf{10.455} \\
% 40 & 75.990 & 44.710 & 40.199 & \bf{40.093} & 21.456 & 21.360 & 12.425 & \bf{12.418} & 23.971 & 21.696 & 15.258 & \bf{15.222} & 13.234 & 11.447 & 10.111 & \bf{10.086} \\
% 60 & 69.947 & 37.561 & 31.891 & \bf{31.784} & 21.429 & 21.297 & 11.194 & \bf{11.187} & 23.899 & 20.409 & 13.749 & \bf{13.743} & 13.217 & 11.408 & 10 & 10 \\
% 80 & 64.154 & 32.580 & 26.094 & \bf{26.073} & 21.417 & 21.176 & 10.476 & \bf{10.474} & 23.763 & 12.798 & 12.654 & \bf{12.574} & 13.188 & 11.385 & 10 & 10 \\
% 100 & 57.170 & 24.959 & 21.926 & \bf{21.899} & 21.395 & 21.056 & 10.013 & \bf{10.012} & 23.757 & 12.711 & 12.138 & \bf{12.129} & 13.070 & 11.324 & 10 & 10 \\
% \bottomrule

% \toprule
% \multirow{2}{*}{\centering b } & \multicolumn{4}{c|}{DBLP (WC model)} & \multicolumn{4}{c|}{Twitter (WC model)} & \multicolumn{4}{c|}{Stanford (WC model)} & \multicolumn{4}{c}{Youtube (WC model)} \\ 
% & RA & OD & AG & GR & RA & OD & AG & GR & RA & OD & AG & GR & RA & OD & AG & GR \\
% \midrule
% 20 & 118.23 & 118.17 & 32.602 & \bf{32.601} & 259.45 & 235.73 & 199.40 & \bf{198.76} & 25.803 & 25.800 & 11.742 & \bf{11.740} & 25.663 & 25.368 & 10.152 & \bf{10.113} \\
% 40 & 118.16 & 117.81 & 18.429 & \bf{18.409} & 258.86 & 226.28 & 170.20 & \bf{168.64} & 25.790 & 25.779 & 10.435 & \bf{10.398} & 25.585 & 25.330 & 10.012 & \bf{10.006} \\
% 60 & 118.09 & 117.73 & 11.869 & \bf{11.867} & 257.75 & 214.90 & 144.61 & \bf{144.23} & 25.777 & 25.771 & 10.119 & \bf{10.101} & 25.446 & 25.149 & 10 & 10 \\
% 80 & 117.97 & 117.59 & 10 & 10 & 255.48 & 204.17 & 129.53 & \bf{128.75} & 25.685 & 25.633 & 10.005 & \bf{10.002} & 25.346 & 25.113 & 10 & 10 \\
% 100 & 117.94 & 117.43 & 10 & 10 & 254.04 & 196.40 & 114.11 & \bf{112.07} & 25.657 & 25.603 & 10.002 & \bf{10.000} & 25.277 & 25.052 & 10 & 10 \\
% \bottomrule
\end{tabular} }
\vspace{-5mm}
\end{table*}

% \vspace{-8mm}
\begin{table*}[!htbp]
\vspace{-4mm}
\centering
\caption{\jiadong{Expected Spread in the IMIN-EB problem (IC model)}}\label{table:heuristics-eb}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|lllll|lllll|lllll|lllll}
\toprule
\multirow{2}{*}{\centering b } & \multicolumn{5}{c|}{EmailCore (TR model)} & \multicolumn{5}{c|}{Facebook (TR model)} & \multicolumn{5}{c|}{Wiki-Vote (TR model)} & \multicolumn{5}{c}{EmailAll (TR model)} \\
& RA & OD & GS & AG & GR & RA & OD & GS & AG & GR & RA & OD & GS & AG & GR & RA & OD & GS & AG & GR \\
\midrule
20 & 364.62$^{***}$ & 364.42$^{***}$ & 362.652$^{**}$& 361.54$^{*}$ & \bf{361.51}
& 57.846$^{***}$ & 58.04$^{***}$ & 33.349$^{*}$ &33.346$^{*}$ & \bf{33.279}
& 484.60$^{***}$ & 487.94$^{***}$ & 167.17$^{**}$ & 167.93$^{**}$ & \bf{166.79}
& 1,567.0$^{***}$ & 1566.2$^{***}$ & 354.67$^{***}$ & 361.51$^{***}$ & \bf{338.46} \\
40 & 364.53$^{***}$ & 364.36$^{***}$ & 356.98$^{*}$ &357.15$^{*}$ & \bf{356.48}
& 57.829$^{***}$ & 57.829$^{***}$ & 23.751$^{*}$ &23.748$^{*}$ & \bf{23.702}
& 481.22$^{***}$ & 482.27$^{***}$ & 41.025$^{**}$ &42.768$^{**}$ & \bf{40.205}
& 1,561.9$^{***}$ & 1564.1 $^{***}$& 82.792$^{***}$ & 83.462$^{***}$ & \bf{81.488} \\
60 & 364.42$^{***}$ & 364.23$^{***}$ & 335.16$^{***}$ &336.62$^{***}$ & \bf{333.41}
& 57.669$^{***}$ & 57.579$^{***}$ & 18.907$^{*}$ & 18.901$^{*}$ & \bf{18.859}
& 480.61$^{***}$ & 482.20$^{***}$ & 16.991$^{*}$ &17.329$^{**}$ & \bf{16.311}
& 1,556.6$^{***}$ & 1561.0$^{***}$ & 25.204$^{**}$& 28.143$^{***}$ & \bf{23.414} \\
80 & 364.30$^{***}$ & 364.10$^{***}$ & 275.15$^{***}$ &281.97$^{***}$ & \bf{267.79}
& 57.568$^{***}$ & 57.363$^{***}$ & 15.631$^{*}$ &15.624$^{*}$ & \bf{15.611}
& 479.28$^{***}$ & 475.20$^{***}$ & 11.489$^{*}$ &11.491$^{*}$ & \bf{11.360}
& 1,556.6$^{***}$ & 1558.2$^{***}$ & 13.049$^{**}$ & 14.049$^{**}$ & \bf{12.954} \\
100 & 364.12$^{***}$ & 363.81$^{***}$ & 197.25$^{***}$ & 206.65$^{***}$ & \bf{189.50}
& 57.322$^{***}$ & 57.316$^{***}$ & 13.329 & 13.330$^{*}$ & {13.329}
& 475.67$^{***}$ & 472.55$^{***}$ & 10.097$^{*}$ &10.101$^{*}$ & \bf{10.086}
& 1,551.9$^{***}$ & 1550.7$^{***}$ & 11.628$^{*}$ & 11.783$^{*}$ & \bf{11.590} \\
\bottomrule
\toprule
\multirow{2}{*}{\centering b } & \multicolumn{5}{c|}{DBLP (TR model)} & \multicolumn{5}{c|}{Twitter (TR model)} & \multicolumn{5}{c|}{Stanford (TR model)} & \multicolumn{5}{c}{Youtube (TR model)} \\
& RA & OD&GS & AG & GR & RA & OD&GS & AG & GR & RA & OD&GS & AG & GR & RA & OD&GS & AG & GR \\
\midrule
20 & 10.690$^{**}$ & 10.692$^{***}$ & 10.448$^{*}$& 10.451$^{*}$ & \bf{10.354}
& 16,800$^{***}$ & 16,800$^{***}$ & 16,703$^{**}$ & 16,701$^{**}$ & \bf{16,697}
& 13.477$^{***}$ & 13.456$^{***}$ & 11.294$^{***}$ & 11.540$^{***}$ & \bf{10.989}
& 10.819$^{**}$ & 10.817$^{**}$ & 10.079$^{*}$ & 10.081$^{*}$ & \bf{10.069} \\

40 & 10.686$^{**}$ & 10.688$^{**}$ & 10.251$^{*}$ & 10.253$^{*}$ & \bf{10.144}
& 16,800$^{***}$ & 16,799$^{***}$ & 16,662$^{***}$ &16,760$^{***}$ & \bf{16,607}
& 13.471$^{***}$ & 13.439$^{***}$ & 10.503$^{*}$ & 10.512$^{*}$ & \bf{10.487}
& 10.803$^{**}$ & 10.817$^{**}$ & 10.030$^{*}$ & 10.031$^{*}$ & \bf{10.025} \\

60 & 10.684$^{*}$ & 10.687$^{**}$ & 10.048$^{*}$ & 10.055$^{*}$ & \bf{10.037}
& 16,799$^{***}$ & 16,799$^{***}$ & 16,581$^{***}$ & 16,588$^{***}$ & \bf{16,567}
& 13.503$^{***}$ & 13.460$^{***}$ & 10.205$^{*}$  & 10.232$^{*}$ & \bf{10.105}
& 10.801$^{**}$ & 10.814$^{**}$ & 10.008$^{*}$ & 10.006$^{*}$ & \bf{10.005} \\

80 & 10.682$^{**}$ & 10.685$^{**}$ & 10.021$^{*}$ & 10.023$^{*}$ & \bf{10.015}
& 16,799$^{***}$ & 16,797$^{***}$ & 15,991$^{***}$ &16,552$^{***}$ & \bf{15,650}
& 13.469$^{***}$ & 13.555$^{***}$ & 10.067$^{*}$ & 10.097$^{*}$ & \bf{10.011}
& 10.800$^{**}$ & 10.804$^{***}$ & 10.001 & 10.002$^{*}$ & {10.001} \\

100 & 10.673$^{**}$ & 10.669$^{**}$ & 10.013$^{*}$ &10.016$^{*}$ & \bf{10.004}
& 16,796$^{***}$ & 16,797$^{***}$ & 13,628$^{***}$ & 16,486$^{***}$ & \bf{11,479}
& 13.518$^{***}$ & 13.453$^{***}$ & 10.012$^{*}$ &  10.040$^{*}$ & \bf{10}
& 10.797$^{**}$ & 10.790$^{**}$ & 10 &10 & 10 \\
\bottomrule


\multicolumn{13}{l}{\begin{minipage}{1.1\textwidth}  Notes. Best performers are bold. All experiments are repeated five times.

~~~~~~~~~~~~~~$^{*}p<0.1$; $^{**}p<0.05$; $^{***}p<0.001$.
\end{minipage}}
\end{tabular} }
\vspace{-5mm}
\end{table*}


\noindent \textbf{Comparison with Other Heuristics.}
% {\color{red} The results are for IMIN problem, not IMIN-EB problem, right?}
\jiadong{As discussed in Section~\ref{sec:advanced-greedy}, the effectiveness (expected spread) of the AG algorithm is the same as the BG algorithm.
% {\color{red}In Section~\ref{sec:advanced-greedy}, there are only two lines about the effectiveness. Is it for sure?}.
Thus, we compare the effectiveness (i.e., expected spread) of our proposed algorithms (AG and GR) with other heuristics (RA, OD and GS) on all networks (EC, F, W, EA, D, T, S, Y) under the IC model using pairwise t-tests in Tables~\ref{table:heuristics} (IMIN problem) and Table \ref{table:heuristics-eb} (IMIN-EB problem). The results under the LT model are included in the Tables A5 and A6 in online appendix. We first randomly select $10$ nodes as the seeds and vary the budget $b$ from $20,40,60,80$ to $100$. We repeat this process by $5$ times and report the average expected spread with the resulting blockers (the expected spread is computed by MCS with $10^5$ rounds). The bold numbers in Table \ref{table:heuristics} and \ref{table:heuristics-eb} denote the minimum expected spread across the four algorithms. The results under the WC model can be found in Table A4 and Table A5.}

The findings indicate that our GR algorithm consistently attains the optimal outcome, characterized by the lowest expected spread, across various budgets and propagation models. The performance of GR algorithm surpasses that of the other algorithms, with improvements that are statistically significant. Moreover, as the budget $b$ increases, the efficacy of the GR algorithm improves.
The findings substantiate the superiority of our proposed algorithm, GR, in terms of effectiveness when compared to other existing algorithms.


% \subsection{Efficiency Comparison}
% In this section, we first compare the efficiency of our proposed algorithms (AG and GR) with state-of-the-art BG algorithms. Then, we demonstrate the scalability of our proposed GR algorithm. 


\noindent \textbf{Time Cost of Different Algorithms.}
\jiadong{We compare the running time of BG, GS, AG, and GR, and set the budget $b$ to $10$ due to the huge computation cost of the BG.
Figures~\ref{fig:time-imin}, A2 and A3 show the results for all networks under the two propagation models where the x-axis denotes different networks and the y-axis is the running times (s) of the algorithms.
For the IMIN problem, the BG algorithm is unable to return results within the specified time constraint of 24 hours for six networks under the TR model, and for five networks under the WC model. For IMIN-EB problem, the BG algorithm does not return any results within 72 hours in all datasets, while the number of candidates of IMIN-EB is much larger than IMIN (the number of edges v.s. the number of nodes).
The results indicate that our proposed algorithms, namely AG and GR algorithms, exhibit significantly better runtime performance compared to existing state-of-the-art BG algorithm. The difference in runtime is at least three orders of magnitude, and this gap tends to be even larger when applied to larger networks. These results align with the analysis of time complexities presented in Section~\ref{sec:advanced-greedy}. Additionally, the time required for GR is similar to that of AG.
We can also observe that the running time of all three algorithms under the LT model is generally smaller than under the IC model. This is likely due to the fact that the sampled graphs in the LT model are smaller, as each node can have at most one in-neighbor.
Additionally, the speedup in running time for the AG and GR algorithms is greater compared to the BG, which can be attributed to the strict linear refinement of these two algorithms under the LT model.}

\begin{figure}[!htbp]
\begin{minipage}{0.49\linewidth}
\begin{subfigure}[h]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/time-b=10-tr.pdf}
    \caption{TR \& IC model in IMIN problem}
    \label{fig:time-tr}
    \end{subfigure}
    % \hspace{1mm}
% \begin{subfigure}[h]{0.48\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-b=10-wc.pdf}
%     \caption{\color{red}WC \& IC model in IMIN problem}
%     \label{fig:time-wc}
%     \end{subfigure}
%     \hspace{1mm}
    \begin{subfigure}[h]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig/time-b=10-tr-edge.pdf}
    \caption{\jiadong{TR \& IC model in IMIN-EB problem}}
    \label{fig:time-tr-eb}
    \end{subfigure}
    % \hspace{1mm}
% \begin{subfigure}[h]{0.48\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-b=10-wc-edge.pdf}
%     \caption{\jiadong{\color{red}WC \& IC model in IMIN-EB problem}}
%     \label{fig:time-wc-eb}
%     \end{subfigure}
    \caption{Time Cost of Different Algorithms} \label{fig:time-imin}
    \end{minipage}
    \begin{minipage}{0.49\linewidth}
    \begin{subfigure}[h]{0.49\linewidth}
\centering
    \includegraphics[width=1\columnwidth]{fig/time-facebook-tr.pdf}
    \caption{TR \& IC model in \texttt{Facebook} dataset}\label{fig:time-budget-a}
\end{subfigure}
% \begin{subfigure}[h]{0.49\linewidth}
% \centering
%     \includegraphics[width=1\columnwidth]{fig/time-facebook-wc.pdf}
%     \caption{\texttt{Facebook} (WC \& IC model)}\label{fig:time-budget-b}
% \end{subfigure}
\begin{subfigure}[h]{0.49\linewidth}
\centering
    \includegraphics[width=1\columnwidth]{fig/time-dblp-tr.pdf}
    \caption{TR \& IC model in \texttt{DBLP} dataset}\label{fig:time-budget-c}
\end{subfigure}
% \begin{subfigure}[h]{0.49\linewidth}
% \centering
%     \includegraphics[width=1\columnwidth]{fig/time-dblp-wc.pdf}
%     \caption{\texttt{DBLP} (WC \& IC model)}\label{fig:time-budget-d}
% \end{subfigure}
%\vspace{-1mm}
\caption{Running Time v.s. Budget in the IMIN problem}
\label{fig:time-budget}
    \end{minipage}
    \vspace{-3mm}
\end{figure}



% \begin{figure}[!htbp]
% \begin{subfigure}[h]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-b=10-tr-edge.pdf}
%     \caption{\jiadong{TR \& IC model}}
%     \label{fig:time-tr-eb}
%     \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-b=10-wc-edge.pdf}
%     \caption{\jiadong{WC \& IC model}}
%     \label{fig:time-wc-eb}
%     \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-b=10-tr-lt-edge.pdf}
%     \caption{\jiadong{TR \& LT model}}
%     \label{fig:time-tr-lt-eb}
%     \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{fig/time-b=10-wc-lt-edge.pdf}
%     \caption{\jiadong{WC \& LT model}}
%     \label{fig:time-wc=lt=eb}
%     \end{subfigure}
%     \caption{\jiadong{Time Cost of Different Algorithms in the IMIN-EB problem}} \label{fig:time-imin-eb}
% \end{figure}


{\color{rehigh}\noindent {\bf Varying the Budget.}
The running time of the algorithms on \texttt{Facebook} and \texttt{DBLP} networks are shown in Figures~\ref{fig:time-budget} and A4 for various budgets.
The running time of AG may decrease with larger budgets due to the early termination (Lines 19-20 in Algorithm~\ref{algo:greedyreplace}).
Our proposed algorithms AG and GR exhibit significantly greater efficiency in comparison to the most advanced existing method BG, with the disparity between them further enlarged as the budget expands. Additionally, it is observed that the computational time required for AG is similar to that of GR. AG may exhibit faster performance than GR in cases where the budget is limited. However, as the budget increases, GR demonstrates superior performance in terms of running time.

%BG under larger budgets in \texttt{Facebook} and under all budgets in \texttt{DBLP} is not shown because it does not return any results within $48$ hours. 


% \begin{figure}[!htbp]
% \centering
% \begin{subfigure}[h]{0.24\linewidth}
% \centering
%     \includegraphics[width=1\columnwidth]{fig/time-facebook-tr.pdf}
%     \caption{\texttt{Facebook} (TR model)}\label{fig:time-budget-a}
% \end{subfigure}
% \begin{subfigure}[h]{0.25\linewidth}
% \centering
%     \includegraphics[width=1\columnwidth]{fig/time-facebook-wc.pdf}
%     \caption{\texttt{Facebook} (WC model)}\label{fig:time-budget-b}
% \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
% \centering
%     \includegraphics[width=1\columnwidth]{fig/time-dblp-tr.pdf}
%     \caption{\texttt{DBLP} (TR model)}\label{fig:time-budget-c}
% \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
% \centering
%     \includegraphics[width=1\columnwidth]{fig/time-dblp-wc.pdf}
%     \caption{\texttt{DBLP} (WC model)}\label{fig:time-budget-d}
% \end{subfigure}
% %\vspace{-1mm}
% \caption{Running Time v.s. Budget in the IMIN problem (IC model)}
% \label{fig:time-budget}
%     \vspace{-1mm}
% \end{figure}

==> imin-eb.tex <==
\section{Approach for IMIN-EB Problem}
\label{sec::app-IMIN-EB}

\subsection{AdvancedGreedy-EB Algorithm}
\label{sec:imin-eb-ag}


\subsection{Approximation Guarantee of Greedy Algorithm}
\label{sec:imin-eb-appro}


\subsection{GreedyReplace-EB Algorithm}
\label{sec:imin-eb-ag}


==> intros.tex <==
\IEEEraisesectionheading{\section{Introduction}
\label{sec:intros}}



\IEEEPARstart{W}{ith} the prevalence of social network platforms such as Facebook and Twitter, a large portion of people is accustomed to expressing their ideas or communicating with each other online. 
%As online platforms provide fast access to large-scale information, and a topic may spread through the connections between individuals. 
Users in online social networks receive not only positive information (e.g., new ideas and innovations) \cite{positive-inf}, but also negative messages (e.g., rumors and fake science) \cite{min-greedy2}. 
In fact, misinformation like rumors spread fast in social networks \cite{rumour-quick}, and can form more clusters compared with positive information \cite{anti-vacc}, which should be limited to avoid `bad' consequences. 
%More than just the rumors, the diffusion of fake science is also dangerous. 
For example, the opposition to vaccination against SARS-CoV-2 (causal agent of COVID-19) can amplify the outbreaks \cite{covid19-2}. The rumor of White House explosions that injured President Obama caused a \$136.5 billion loss in the stock market~\cite{fakenews}. %covid19-1,
Thus, it is critical to efficiently minimize the influence spread of misinformation. %negative influence minimization problem.

We can model the social networks as graphs, where vertices represent users and edges represent their social connections. The influence spread of misinformation can be modeled as the expected spread under diffusion models, e.g., the independent cascade (IC) model~\cite{first-max}.
The strategies in existing works on spread control of misinformation can be divided into two categories: (i) blocking vertices \cite{min-greedy1,min-greedy-tree, FanLWTMB13, Nature-error, Viruses}, which usually removes some critical users in the networks such that the influence of the misinformation can be limited; or blocking edges \cite{min-edge1,min-edge2,WangDLYJY20}, which removes a set of edges to stop the influence spread of misinformation; (ii) spreading positive information \cite{min-greedy2,LeeSMH19,seed-positive,HeSCJ12}, which considers amplifying the spread of positive information to fight against the influence of misinformation.

In this paper, we consider blocking key vertices in the graph to control the spread of misinformation.
Suppose a set of users are already affected by misinformation and they may start the propagation, we have a budget for blocking cost, i.e., the maximum number of users that can be blocked.
Then, we study the influence minimization problem \cite{min-greedy1,min-greedy-tree}: given a graph $G$, a seed set $S$ and a budget $b$, find a blocker set $B^*$ with at most $b$ vertices such that the influence (i.e., expected spread) from $S$ is minimized. Note that blocking vertices is the most common strategy for hindering influence propagation. For example, in social networks, disabling user accounts or preventing the sharing of misinformation is easy to implement. According to the statistics, Twitter has deleted 125,000 accounts linked to terrorism~\cite{twitter-delete}.
Obviously, we cannot block too many accounts, it will lead to negative effect on user experience. In such cases, it is critical to identify a user set with the given size whose blocking effectively hinders the influence propagation.

% Previous works show that the strategy of removing vertices in decreasing order of out-degree can often be effective \cite{Nature-error,Viruses}. However, later works find the greedy algorithm is more effective than the out-degree \cite{min-greedy1,min-greedy-tree}. 
%Ans the experiments show our MOVE algorithm has better performance than greedy algorithm. Besides, if we take into account the issue of user experience and the limitations of the cost, we need a budget, i.e., the maximum number of users that can be blocked.

%Most existing works need the budget as the input, as they assume the budget is already known \cite{min-greedy-tree,min-greedy1}. However, many real-life applications aim to keep the most users in the social network safe from the negative information, e.g., keep $90\%$ of the users not be affected by the negative information. In such scenarios, the budget is flexible, and the goal is to minimize the budget used to keep most users not active by the negative information. Motivated by this, we define the \underline{B}udget \underline{M}inimization with \underline{D}eclining \underline{R}atio \underline{G}uarantee (BM-DRG) Problem, which aims to minimize the budget for blocking users while $\eta$ of users who are affected by negative information will be safe. while the cooperation among the candidate blockers is not considered

\vspace{1mm}
\noindent \textbf{Challenges and Existing Solutions.}
The influence minimization problem is NP-hard and hard to approximate, and we are the first to prove them (Theorems~6 and~9).
Due to the hardness of the problem, the state-of-the-art solutions use a greedy framework to select the blockers \cite{min-greedy1,min-greedy2}, which outperforms other existing heuristics \cite{min-greedy-tree,Nature-error,Viruses}.
However, different to the influence maximization problem, the spread function of our problem is not supermodular (Theorem~8), which implies that an approximation guarantee may not exist for existing greedy solutions.
%Another major challenge is that existing works use Monte-Carlo Simulations to compute the influence spread, which is cost-prohibitive on large graphs even for light heuristics.
%Moreover, as discussed in Section~\ref{sec:ec-exist}, the reverse influence sampling (RIS) technique is feasible to directly apply to our problem, as the reverse is no need for our computation of expected spread decreasing for each candidate blocker.
\revise{Moreover, as the computation of influence spread under the IC model is \#P-hard~\cite{maximization1}, the state-of-the-art solutions use Monte-Carlo Simulations to compute the influence spread.
However, such methods are cost-prohibitive on large graphs since there are excessive candidate blockers and they have to compute the decrease of expected spread for every candidate blocker (detailed in Section~\ref{sec:ec-exist}).}

%enumerate all the candidate blockers and compute the expected spread decreasing when blocking each of them.

\vspace{1mm}
\noindent \textbf{Our Solutions.}
\revise{
Different to the state-of-the-art solutions (the greedy algorithms with Monte-Carlo Simulations), we propose a novel algorithm (GreedyReplace) based on sampled graphs and their dominator trees.
Inspired by reverse influence sampling \cite{Borgs-max}, the main idea of the algorithm is to simultaneously compute the decrease of expected spread of every candidate blocker, which uses almost a linear scan of each sampled graph.
We prove that the decrease of the expected spread from a blocked vertex is decided by the subtrees rooted at it in the dominator trees that generated from the sampled graphs (Theorem~\ref{theo:dominator-subtree}).
Thus, instead of using Monte-Carlo Simulations, we can efficiently compute the expected spread decrease through sampled graphs and their dominator trees.} 
We also prove the estimation ratio is theoretically guaranteed given a certain number of samples (Theorem~\ref{theorem:approx}). 
Equipped with above techniques, we first propose the AdvancedGreedy algorithm, which has a much higher efficiency than the state-of-the-art greedy method without sacrificing its effectiveness.
%Due to the huge computation cost of Monte-Carlo Simulations and the inspiration from reverse influence sampling \cite{Borgs-max}, 

Furthermore, for the vertex blocking strategy, we observe that all out-neighbors of the seeds will be blocked if the budget is unlimited, while the greedy algorithm may choose the vertices that are not the out-neighbors as the blockers and miss some important candidates. {We then propose a new heuristic, named the GreedyReplace algorithm, focusing on the relationships among candidate blockers: we first consider blocking vertices by limiting the candidate blockers in the out-neighbors, and then try to greedily replace them with other vertices if the expected spread becomes smaller.}


\vspace{1mm}
\noindent \textbf{Contributions.}
Our principal contributions are as follows.

\begin{itemize}

\item %Motivated by the existing studies, we explore the Influence Minimization problem to minimize the influence of misinformation by blocking key vertices.
   %calculate the minimal expected spread for controlling the negative influence propagation under a given budget.
     We are the first to prove the Influence Minimization problem is NP-hard and APX-hard unless P=NP. %The problem is shown to be more challenging than the influence maximization problem whose objective function is submodular.
     
\item 

\revise{
We propose the first method to estimate the influence spread decreased by every candidate blocker under IC model, which only needs a simple scan on the dominator tree of each sampled graph.  
We prove an estimation ratio is guaranteed given a certain number of sampled graphs.
To the best of our knowledge, we are the first to study the dominator tree in influence related problems.
%an advanced greedy algorithm based on the sampled graphs and dominator tree, which can
}

%\item Our advanced greedy algorithm is proposed to accelerate the runtime of the state-of-the-art greedy algorithm with the same effectiveness.
% \item We propose the Iterative Progress (IP) algorithm to quickly compute an accurate influence spread, which iteratively converges the activation probability of each vertex to the optimal value. A maintenance mechanism is introduced to update the activation probabilities against graph changes. We show that the IP algorithm can be used in other problems related to computing expected influence spread. % on IC model.
    
\item  \revise{Equipped with the above estimation technique, our AdvancedGreedy algorithm significantly outperforms the state-of-the-art greedy algorithms in efficiency without sacrificing effectiveness. We also propose a superior heuristic, the GreedyReplace algorithm, to further refine the effectiveness. }

% which considers the relationships among candidate blockers. It also combines the advantages of the greedy method and the blocking on seed neighbors by greedily replacing the blockers if the expected spread becomes smaller.
%combine the advantages of the greedy algorithm and the blocking on the close neighbors of the seed vertices.
%by greedily replacing the blockers if the expected spread becomes smaller.


\item Comprehensive experiments on $8$ real-life datasets validate that our AdvancedGreedy algorithm is faster than the state-of-the-art (the greedy algorithm with Monte-Carlo Simulations) by more than $3$ orders of magnitude, and our GreedyReplace algorithm can achieve better result quality (i.e., the smaller influence spreads) and close efficiency compared with our AdvancedGreedy algorithm. %Even more, the experiments show our GreedyReplace algorithm also has superior on efficiency when budget increases.
\end{itemize}

==> intros_MS.tex <==
\section{Introduction}\label{sec:intros}

\jiadong{
In today's hyper-connected world, the concept of influence maximization, which aims to target a select group of individuals in order to maximize the spread of influence \citep{value-customer, first-max}, has long been a focal point of research due to its commercial potential in various industries such as marketing, finance, education, etc \citep[e.g.,][]{maximization1, banerjee2013diffusion, gunnecc2020least, wu2020diffnet++,raghavan2022influence,eckles2019seeding,zhou2023detecting,TengXZWZ23}. However, a lesser-explored yet equally critical counterpart to this problem is the \emph{influence minimization} problem. This problem involves identifying a specific set of nodes (or edges) in a network in order to minimize the spread of influence, particularly when some forms of influence are detrimental. Let us provide the following two examples to illustrate the importance of minimizing the spread of influence.}
% and visually illustrate our solution to the problem in Figure~\ref{fig:melcup-road}.

% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}[h]{0.24\linewidth}
% \includegraphics[width=1\columnwidth]{fig/melcup-0(2).jpg}
%     \caption{Initial}\label{fig:melcup-0}
% \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
%     \includegraphics[width=1\columnwidth]{fig/melcup-100(2).jpg}
%     \caption{Blocking $100$ Nodes}\label{fig:melcup-100}
% \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
%     \includegraphics[width=1\columnwidth]{fig/road-0.jpg}
%     \caption{Initial}\label{fig:road-1}
% \end{subfigure}
% \begin{subfigure}[h]{0.24\linewidth}
%     \includegraphics[width=1\columnwidth]{fig/road-50.jpg}
%     \caption{Blocking $50$ Nodes}\label{fig:road-2}
% \end{subfigure}
% \begin{minipage}{\textwidth}\footnotesize  Notes: Figures \ref{fig:melcup-0} and \ref{fig:melcup-100} illustrate our proposed approach for reducing information dissemination on the Twitter platform. Figures \ref{fig:road-1} and \ref{fig:road-2} illustrate our proposed solution for reducing the spread of influence on the road network in Minnesota. \end{minipage}

%     \caption{Demostration of our Proposed Solution for Minimizing Influence Propagation}
%     \label{fig:melcup-road}
%     \vspace{-2mm}
% \end{figure*}

\noindent
\jiadong{
\textbf{Reducing Misinformation Propagation.} In the era of rapid information dissemination and the prevalence of social media, the proliferation of misinformation has emerged as a major societal concern and is regarded as one of the most significant global economic risks \citep{WEF2022}. The dissemination of false information or unverified rumors can lead to various adverse effects, such as economic damage, substantial disruption, and widespread panic. For example, a false tweet claiming that Barack Obama was injured in an explosion at the White House led to a significant decline of \$136.5 billion in the stock market~\citep{fakenews}. 
% In fact, misinformation, such as rumors, spreads faster than true news in social networks \citep{vosoughi2018spread} and tends to form more clusters than positive information \citep{anti-vacc}. 
Therefore, it is crucial to identify influential nodes or edges within the social network to restrict the dissemination of such misinformation and mitigate the potential negative consequences.}
% Figure~\ref{fig:melcup-0} illustrates an example of influence propagation on Twitter~\citep{ZhangZYPN19}, where the shade of red represents the probability of users being influenced.
% As shown in Figure~\ref{fig:melcup-100}, we observed a significant decrease in the expected spread of propagation by blocking $100$ key nodes using our proposed methods.

\noindent \jiadong{\textbf{Enhancing Epidemic Control.} The outbreak of infectious diseases poses formidable challenges to public health systems worldwide, demanding swift and strategic intervention to limit transmission. 
% The emergence and rapid spread of infectious agents can swiftly overwhelm healthcare infrastructures, jeopardizing the health and well-being of communities on a global scale. 
For example, COVID-19 is being attributed as the final factor leading to the breakdown of the United Kingdom's healthcare system \citep{mclellan2022nhs}. In such scenarios, timely responses become paramount to mitigate the potential cascading effects on morbidity, mortality, and socio-economic stability. The adverse effects of infectious disease outbreaks underscore the importance of harnessing innovative solutions that can efficiently identify critical nodes or edges within transmission networks and guide swift containment measures.}
% As an illustration, Figure~\ref{fig:road-1} is a visual demonstration of the propagation of influence on the Minnesota road network when $100$ nodes are randomly selected as seeds.\footnote{\url{http://www.cise.ufl.edu/research/sparse/matrices/Gleich/minnesota}}
% Darker shades of red signify a greater likelihood of influence. The results shown in Figure~\ref{fig:road-2} demonstrate that blocking a set of $50$ nodes selected by our proposed method significantly hinders the spread of influence.

\jiadong{
The above examples highlight the urgent need for effective solutions to the influence minimization problem. The problem can be formulated as follows \citep{min-greedy1}: a social network (or a transmission network) is modeled as a graph where nodes represent individuals and edges represent connections or relationships between them. The propagation of influence (e.g., fake news or diseases) in a network follows a diffusion model, such as the \emph{independent cascade} (IC) model or \emph{linear threshold} (LT) model~\citep{first-max}. Given a graph $G$, a seed set $S$, and a budget $b$, the objective of the influence minimization problem is to identify a set $B^*$ consisting of at most $b$ nodes (or $b$ edges) that minimizes the expected number of nodes activated by the seeds $S$ (referred to as the expected influence spread) under a specific diffusion model.}

\jiadong{
Existing research has explored various methods to tackle the influence minimization problem \citep[e.g.,][]{min-edge1,min-greedy1, min-edge2,min-greedy-tree}. However, a common limitation observed in these approaches is their high time complexity. For instance, the processing time required for the Wiki-Vote network (7K nodes and 103K edges) exceeds three days when using these methods. This significantly hinders their applicability to large networks and real-time scenarios where prompt decision-making is essential for effective intervention \citep{DBLP:journals/jnca/ZareieS21}. From a pragmatic perspective, it is impractical for an algorithm to require a longer duration to discover a solution that minimizes influence spread compared to the actual time required for influence to propagate. }

\jiadong{
To address the limitation, we present novel and efficient algorithms that tackle the influence minimization problem. Our algorithms address the scalability issues encountered by existing solutions, providing a significant leap forward in terms of computational speed and adaptability to large-scale real-world networks. Our proposed algorithms showcase an unprecedented speedup, outperforming existing methods by an astonishing three orders of magnitude. In addition, we conduct an exhaustive series of real-data experiments to evaluate the efficacy and applicability of our proposed algorithms in a variety of scenarios. In the following section, we discuss the various technical challenges encountered and the corresponding contributions in detail.}

\vspace{1mm}
\noindent \textbf{Main Technical Challenges.}
\jiadong{
There are several technical challenges in influence minimization problems. First, the influence minimization problem is NP-hard under both node blocking and edge blocking strategies with the IC/LT influence propagation model (Theorems~6 and 7). Then, the state-of-the-art algorithms employ a greedy framework to select the blockers \citep{min-greedy1,min-greedy2}, which has proven to be superior to alternative heuristics proposed in previous studies \citep[e.g,][]{Nature-error,Viruses,min-greedy-tree}. However, in contrast to the influence maximization problem, we demonstrate that the expected spread function in the influence minimization problem does not exhibit supermodularity (Theorem~8). As a result, existing greedy solutions may not possess an approximation guarantee.}
% We also prove that the expected spread function is supermodular for the LT model (Theorem~10), such that the greedy algorithm can achieve a $(1-1/e-\epsilon)-$approximation.
% {\color{red} TODO - I see that in theorem 10, the expected spread function is supermodular for LT model. So can we still say this?}

\jiadong{Second, similar to the influence maximization problem, an essential component of the greedy algorithm involves the computation of the influence spread from the seeds, a problem known to be \#P-hard~\citep{maximization1}. Rather than relying on an exact algorithm, state-of-the-art solutions for estimating influence spread in diffusion models utilize Monte-Carlo Simulations \citep{influencepath,OhsakaAYK14,MS-PCG}.
% r {\color{red}Reverse Influence Sampling \citep{SunHYC18,Guo0WC20} Should I add RIS?}.
In contrast to the influence maximization problem, the influence minimization problem incorporates an additional step, which involves the computation of the reduction in expected influence spread that would occur by blocking a particular node or edge (detailed in Section~\ref{sec:ec-exist}). In order to accomplish this, the current algorithms must iterate through all potential nodes or edges. Given the presence of an overwhelming number of potential candidate nodes or edges that could be blocked, the implementation of these methods becomes economically unfeasible when applied to larger graphs.}

\vspace{1mm}
\noindent \textbf{Our Contributions.}
\jiadong{
In this paper, we prove that the influence minimization problem is NP-hard under different blocking strategies (node blocking or edge blocking) with various influence propagation models (IC or LT). For the problem under the LT model, we find that the expected spread function is supermodular, which enables us to leverage the greedy algorithm to achieve a $(1-1/e-\epsilon)$-approximation.}
% {\color{red} TODO - What does this imply? The greedy algorithms may have intrinsic difficulties to be made scalable for large graphs?}
\jiadong{We then tackle the issue of scalability by introducing a novel algorithm, namely the AdvancedGreedy algorithm. This algorithm exhibits a remarkable increase in speed by several orders of magnitude compared to all preexisting greedy algorithms while maintaining their efficacy. The efficiency of our algorithm is enhanced through the simultaneous computation of the expected influence spread reduction for each candidate node {and edges}. This is achieved by employing an almost linear scan of each sampled graph.
{The central concept underlying our algorithm is the utilization of the dominator tree for the computation of the expected reduction in expected influence spread. This novel approach has not yet been employed in the context of influence-related problems.} We prove that the decrease of the expected influence spread from a blocked node is decided by the subtrees rooted in the dominator trees that are generated from the sampled graphs (Theorem~\ref{theo:dominator-subtree}), and we establish that the edge version problem can be effectively solved by transforming it into the node version problem (Theorems~\ref{theo::edge_expected} and \ref{theo:edge-dominator-subtree}).
Hence, rather than relying on Monte Carlo Simulations, we can effectively calculate the expected reduction in influence spread by employing sampled graphs and their dominator trees. We also prove the estimation result is theoretically guaranteed given a certain number of samples (Theorem~\ref{theorem:approx}). Furthermore, we prove the AdvancedGreedy algorithm can achieve a $(1-1/e-\epsilon)$-approximation for both node and edge blocking problems under the LT model.}

\jiadong{
In addition, for the problem under the IC model, since the problem is hard to approximate, we further propose a novel heuristic. When employing the node-blocking strategy, it is evident that if the budget is unlimited, all out-neighbors of the seeds will be blocked. However, the current greedy algorithm may select nodes that are not the out-neighbors as blockers, potentially overlooking crucial candidates. Considering this, we propose a new heuristic, named GreedyReplace algorithm, based on identifying the relationships among candidate blockers. Specifically, we begin by restricting the pool of candidate blockers to the out-neighbors of the blocking nodes. Subsequently, we adopt a greedy strategy to replace these blockers with alternative nodes, should the expected influence spread diminish. This algorithm demonstrates superior performance. }

\jiadong{
We conduct extensive experiments on $8$ real-life publicly available datasets with varying scales, features, and diffusion models. Our proposed algorithms are compared with the state-of-the-art algorithm, namely the greedy algorithm with Monte-Carlo Simulations \citep{min-greedy2,min-greedy1,min-greedy-tree}, as well as other heuristics. Our experiments show that (a) our AdvancedGreedy algorithm exhibits significantly enhanced speed when compared to existing algorithms, surpassing them by a factor of more than three orders of magnitude, (b) our GreedyReplace algorithm demonstrates superior effectiveness, as evidenced by its ability to achieve smaller influence spreads while maintaining comparable efficiency to our AdvancedGreedy algorithm. Our algorithms demonstrate remarkable scalability, enabling it to easily apply to networks comprising millions of nodes and edges.}

% {\color{red} If we do not include demos, remove this paragraph.}
% To further illustrate the versatility and applicability of our algorithms, we provide two compelling demos in Section xx. The first demo showcases how our algorithm can be employed to prevent the spread of fake news on Twitter, a social media platform notorious for its rapid information diffusion. By identifying and blocking influential nodes efficiently, we can disrupt the dissemination of misinformation and mitigate its potentially harmful effects. The second demo illustrates how our approach can be leveraged for effective epidemic control on a road network. Given the pressing global challenges posed by infectious diseases, our algorithm's ability to rapidly identify critical nodes for containment can play a pivotal role in limiting the contagion's spread, ultimately saving lives and mitigating the impact on healthcare systems.

\jiadong{Overall, our research makes significant strides in the realm of influence minimization problems, providing innovative solutions that overcome existing limitations. Our proposed algorithms outperform existing methods by several orders of magnitude in terms of speed. By achieving such remarkable computational efficiency, our approach opens new avenues for managing large-scale networks and real-time scenarios, enabling faster and more proactive responses to potential crises.}


\jiadong{
The remainder of this paper is structured as follows: In Section \ref{sec:relate}, we present a comprehensive review of the related literature. Section \ref{sec:pre} offers a formal definition of the influence minimization problem, introduces the most advanced existing algorithm, and establishes the NP-hard nature of the influence minimization problem. Section \ref{sec::decrease_spread} provides a detailed description of how we calculate the reduction of expected influence spread. Section \ref{sec::app-IMIN} introduces our proposed algorithms and their implementation. Section \ref{sec:exp} outlines the experiment and presents the results obtained from applying our approach to real-life graphs. 
% {\color{red}Section 8 demonstrates the two real-world applications.}
Finally, Section \ref{ses:conclusion} concludes this work, summarizing the main contributions and discussing future research directions.}

A preliminary study of this paper~\citep{0002ZW0023} was presented in the Proceedings of 39th IEEE International Conference on Data Engineering (IEEE ICDE 2023), which only focuses on the problem under the node blocking strategy and the IC model.

==> relat.tex <==
\section{Related Work}
\label{sec:relate}

\noindent \textbf{Influence Maximization.}
The studies of influence maximization are surveyed in~\cite{DBLP:journals/computing/AghaeeGBBF21,DBLP:journals/kais/BanerjeeJP20,DBLP:journals/tkde/LiFWT18}.
Domingos et al. first study the influence between individuals for marketing in social networks \cite{value-customer}. Kempe et al. first model this problem as a discrete optimization problem \cite{first-max}, named Influence Maximization (IMAX) Problem. They introduce the independent cascade (IC) and linear threshold (LT) diffusion models, and propose a greedy algorithm with $(1-1/e)$-approximation ratio since the function is submodular under the above models. Borgs et al. propose a different method based on the reverse reachable set for influence maximization under the IC model \cite{Borgs-max}. Tang et al. propose an algorithm based on martingales for IMAX problem, with a near-linear time cost \cite{max-sota}. %Narayanam et al. study the $\lambda$ Coverage Problem \cite{max-ratio} to find the smallest set such that at least $\lambda$ number of nodes will be activated at the end of diffusion process.

\vspace{1mm}
\noindent \textbf{Influence Minimization.}
Compared with IMAX problem, there are fewer studies on controlling the spread of misinformation, as surveyed in~\cite{DBLP:journals/jnca/ZareieS21}.
Most works consider proactive measures (e.g., blocking nodes or links) to minimize the influence spread, motivated by the feasibility on structure change for influence study \cite{struct-sn,experience-min1,user-attribute2}. %user-attribute1,
In real networks, we may use a degree based method to find the key vertices \cite{Nature-error,Viruses}.
Yao et al. propose a heuristic based on betweenness and out-degree to find approximate solutions \cite{YaoSZWG15}.
Wang et al. propose a greedy algorithm to block a vertex set for influence minimization (IMIN) problem under IC model \cite{min-greedy1}.
Yan et al. also propose a greedy algorithm to solve the IMIN problem under different diffusion models, especially for IC model \cite{min-greedy-tree}. 
They also introduce a dynamic programming algorithm to compute the optimal solution on tree networks. 
The above studies on the IMIN problem validate that the greedy heuristic is more effective than other methods, e.g., degree based heuristics \cite{min-greedy1,min-greedy-tree}.

Kimura et al. propose to minimize the dissemination of negative information by blocking links (i.e., finding $k$ edges to remove) \cite{min-edge1}. They propose an approximate solution for rumor blocking based on the greedy heuristic.
Other than IC model, the vertex and edge interdiction problems were studied under other diffusion models: \cite{min-edge2,NguyenCVD20,KhalilDS14} consider the LT (Linear Threshold) model, \cite{TongPEFF12} considers the SIR (Susceptible-Infected-Recovery) model and \cite{MedyaSS22,abs-1901-02156} considers CD (Credit Distribution) Model.

In addition, there are some other strategies to limit the influence spread. Budak et al. study the simultaneous spread of two competing campaigns (rumor and truth) in a network \cite{min-greedy2}. They prove this problem is NP-hard and provide a greedy algorithm which can be applied to the IMIN problem.
Manouchehri et al. then propose a solution with theoretically guaranteed for this problem~\cite{ManouchehriHD21}.
Moreover, Chen et al. propose the profit minimization of misinformation problem, which not only considers the number of users but also focus on interaction effects between users. As interaction effects are different between different users and the related profit obtained from interaction activities may also be different \cite{ChenLFGD19}.
Lee et al. also consider that both positive and negative opinions are propagating in a social network. Their strategy is to reduce the positive influence near the steady vertices and increase the influence in the vacillating region \cite{LeeSMH19}.
Tong et al. propose the rumor blocking problem to find $k$ seed users to spread the truth such that the user set influenced by the rumor is minimized \cite{seed-positive}.
Some works consider more factors into the propagation models, e.g., user experience~\cite{experience-min1}, evolution of user opinions~\cite{SaxenaHLCNT20}.

In this paper, we consider two different strategies for minimizing influence propagation: vertex blocking (IMIN problem) and edge blocking (IMIN-EB problem), which are two fundamental influence minimization problems.
We first focus on an efficient computation without sacrificing the effectiveness compared with the state-of-the-art and prove it has an approximate guarantee under the LT model. We also further improve the quality of results by proposing a new heuristic for choosing the blockers under the IC model.



\vspace{1mm}
\noindent \textbf{Influence Expected Spread Computation.}
The computation of expected spread is proved to be \#P-hard under IC model \cite{maximization1}. 
Maehara et al. propose the first algorithm to compute influence spread exactly under the IC model \cite{MaeharaSI17}, but it can only be used in small graphs with a few hundred edges. 
Domingos et al. first propose to use the Monte-Carlo Simulations (MCS) to compute the expected spread \cite{first-max}, which repeats simulations until a tight estimation is obtained.
We have to repeatedly run MCS to compute the decrease of influence spread for each candidate blocker, which leads to a large computation cost. 
Borgs et al. propose Reverse Influence Sampling (RIS) \cite{Borgs-max}, which is now widely used in IMAX Problem. Tang et al. then propose the methods to reduce the number of samples for RIS \cite{max-sota}. However, as in our later discussion, we find that RIS is not applicable to our problem (Section~\ref{sec:ec-exist}). 
%As Monte-Carlo Simulations have to compute the spread decrease repetitively for each candidate blocker.
Our one-time computation of the expected spread on sampled graphs can return the spread decrease of every candidate blocker, which avoids redundant computations compared with MCS.



%is based on the sample graph which is the same as Monte-Carlo Simulations theoretically, but our solution can efficiently compute the decrease of expected spread led by each of all vertices at once.

==> relates_MS.tex <==
\section{\rehigh{Related Works}}
\label{sec:relate}
% \rehigh{This section provides an overview of three streams of literature that are relevant to our research. }

\noindent \rehigh{\textbf{The Influence Maximization Problem.}
There are many studies of influence maximization
% The studies of influence maximization are surveyed 
\citep{DBLP:journals/kais/BanerjeeJP20,DBLP:journals/computing/AghaeeGBBF21}.
Domingos and Richardson are the first to study the influence between individuals for marketing in social networks \citep{value-customer}. 
Later, this problem was formulated as a discrete optimization problem, referred to as the influence maximization problem \citep{first-max}.
% ~\cite{first-max} initially formulate this problem as a discrete optimization problem, referred to as the influence maximization problem. 
They introduce the IC and LT diffusion models and propose a greedy algorithm that achieves a $(1-1/e)$-approximation ratio due to the submodularity of the function under these models.
Subsequently, some researchers have proposed advanced approaches, such as reverse sampling \citep{Borgs-max}.
% and stochastic seeding strategies \citep{chin2022evaluating}.
Other researchers have explored strategies to maximize influence in practical scenarios that may involve domain-specific challenges, e.g., costly network information \citep{eckles2019seeding}, user countering \citep{XieCCZLT24}.}
% partial feedback \citep{tang2020influence},
% minimum total amount of inducements \citep{han2019best,gunnecc2020least}, 
% % variations in time horizons \citep{mallipeddi2022framework}, 
% % capacity constraints \citep{DBLP:conf/kdd/0004HSLX023},
% etc.}

% \cite{Borgs-max} propose a novel method for influence maximization based on reverse sampling.
% After that, reverse sampling is widely adopted by subsequent works \cite{max-rr,max-sota}.
% \cite{chin2022evaluating} propose a new random seeding strategy based on the friendship paradox, by seeding the one-hop neighbors of randomly chosen individuals, who are expected to have more friends on average.
% Recently, several studies have explored the application of influence maximization in real-world scenarios, e.g., \cite{eckles2019seeding} focuse on seeding vertices in a network without having complete knowledge of the network, \cite{raghavan2022influence} examine the situation where direct influence has a significant impact, \cite{yadav2017influence} explore maximizing HIV awareness in social networks of homeless youth, \cite{mallipeddi2022framework} develope a data-driven optimization framework to assist firms in conducting successful influencer marketing campaigns.

% {\color{red} TODO - Add what these studies have done: \cite{ eckles2019seeding,yadav2017influence,gunnecc2020least, raghavan2022influence, chin2022evaluating, mallipeddi2022framework}. Some of them are from papers in the business area.}

\rehigh{In contrast to prior research, the objective of this paper is to contribute to the influence minimization problem field, which presents unique challenges that cannot be addressed using existing solutions for influence maximization problem. While the influence minimization problem may appear to be the inverse of the influence maximization problem, it actually entails additional complexities. Specifically, it requires the estimation of the expected reduction in influence spread resulting from the blocking of nodes or edges.}
% This additional step adds further challenges to the problem.}

\noindent \rehigh{\textbf{The Influence Minimization Problem.}
Compared with the influence maximization problem, there are fewer studies on minimizing the spread of influence \citep{DBLP:journals/jnca/ZareieS21}. In general, there are two main strategies that can be employed to solve the influence minimization problem. The first strategy involves blocking (or removing) specific nodes or edges to minimize the overall impact of influence \citep[e.g.,][]{min-edge1,min-greedy1,YaoSZWG15,min-greedy-tree}. The second strategy, known as the counterbalance strategy, involves the dissemination of positive information throughout the network \citep[e.g.,][]{min-greedy2,LeeSMH19,seed-positive,ManouchehriHD21}. By increasing people's awareness and providing them with positive content, the negative influence is reduced. This methodology is predominantly employed to address the dissemination of misinformation. Our papers is the first category.}

\rehigh{Motivated by the feasibility of structure change for influence-related studies \citep{struct-sn,experience-min1,user-attribute2}, most works have focused on utilizing the blocking strategy (i.e., blocking nodes or edges) to minimize the influence spread. Intuitively, simple heuristics that rely on network structure can be employed to identify influential nodes to restrict the spread of influence. For instance, one commonly used heuristic is the degree-based heuristic \citep{Nature-error,Viruses,shah2011rumors,shah2016finding}.
% Another approach involves considering the betweenness and out-degree heuristics \citep{YaoSZWG15}.
However, subsequent studies have shown that these simple degree-based heuristic methods are comparatively less effective than greedy heuristics \citep{min-greedy1,min-greedy-tree}. Hence, different greedy algorithms have been proposed to address the influence minimization problem by blocking nodes or edges under various diffusion models \citep{min-edge1,min-greedy1,min-edge2,min-greedy-tree}.}

% \cite{min-edge1} propose an approximate solution for rumor blocking by blocking edges based on the greedy heuristic. \cite{min-greedy1} propose a greedy algorithm to block a node set for the influence minimization problem under IC model. \cite{min-greedy-tree} also propose a greedy algorithm to solve the influence minimization problem under different diffusion models. They also introduce a dynamic programming algorithm to compute the optimal solution on tree networks. 
% Other than IC model, the node and edge interdiction problems were also studied under Linear Threshold model \citep{min-edge2,NguyenCVD20,KhalilDS14}.

% {\color{red}TODO: If you do not use these diffusion models in the paper, do not mention them from the perspective of the diffusion model. Try to add them to the above paragraphs. }
% Other than IC model, the node and edge interdiction problems were studied under other diffusion models: Linear Threshold model \citep{min-edge2,NguyenCVD20,KhalilDS14}, Susceptible-Infected-Recovery) model \citep{TongPEFF12}  and Credit Distribution Model \citep{MedyaSS22,abs-1901-02156} .

\rehigh{However, a prevalent constraint observed in these methodologies is their limited ability to scale effectively when applied to large networks \citep{DBLP:journals/jnca/ZareieS21}. Even the most advanced greedy approach requires the enumeration of all candidate nodes to calculate the reduction in expected influence spread. Consequently, the computational speed of their solutions often falls short in dealing with real-time scenarios, where quick decisions are crucial for successful intervention. In this paper, we develop a computationally efficient approach that maintains its effectiveness when compared to existing algorithms for minimizing influence spread. Specifically, we consider two fundamental blocking strategies: node blocking and edge blocking. Besides, we also consider two distinct diffusion models, namely the LT model and the IC model.}

\noindent \rehigh{\textbf{The Computation of the Expected Spread.}
An essential aspect of the influence minimization problem involves the estimation of the expected spread, which has been proved to be \#P-hard under IC model \citep{maximization1}. 
Researchers first propose to use the Monte-Carlo Simulations (MCS) to compute the expected influence spread, which repeats simulations until a tight estimation is obtained \citep{first-max}. In a subsequent study \citep{Borgs-max}, researchers propose Reverse Influence Sampling (RIS). Additionally, researchers propose the first algorithm to compute the exact influence spread under the IC model \citep{MaeharaSI17}. However, its applicability is limited to small graphs containing a few hundred edges.
% \cite{first-max} first propose to use the Monte-Carlo Simulations (MCS) to compute the expected influence spread, which repeats simulations until a tight estimation is obtained. In a subsequent study, \cite{Borgs-max} propose Reverse Influence Sampling (RIS). Additionally, \cite{MaeharaSI17} propose the first algorithm to compute the exact influence spread under the IC model. However, its applicability is limited to small graphs containing a few hundred edges.
}

\rehigh{However, as discussed later in Section~\ref{sec:baseline}, we find that {MCS and RIS} are not applicable to our problem. This is because influence minimization problems require repetitive computation of the expected decrease in influence spread for each potential blocked node/edge. We contribute to this stream of literature by introducing the dominator tree when calculating the reduction of expected influence spread, which has not been previously applied to this type of problem.
The dominator tree has predominantly been applied in various fields, e.g., program analysis~\citep{reif1978symbolic,chen2023synthdb} and software testing~\citep{Agrawal99}, which is based on theoretical network flow problems. We, on the other hand, leverage its tree structure properties for our problem, enabling simultaneous estimation of spread reduction across all candidate nodes/edges. This approach minimizes redundant computations in contrast to MCS or RIS methods.
% Our computation of the expected influence spread on sampled graphs can return the spread decrease of every candidate node/edge simultaneously, which avoids redundant computations compared with MCS or RIS.
}


%is based on the sample graph which is the same as Monte-Carlo Simulations theoretically, but our solution can efficiently compute the decrease of expected spread led by each of all nodes at once.
